Channel-Imposed Fusion: A Simple yet Effective Method for Medical Time Series Classification

The automatic classification of medical time series signals, such as electroencephalogram (EEG) and electrocardiogram (ECG), plays a pivotal role in clinical decision support and early detection of diseases. Although Transformer based models have achieved notable performance by implicitly modeling temporal dependencies through self-attention mechanisms, their inherently complex architectures and opaque reasoning processes undermine their trustworthiness in high stakes clinical settings. In response to these limitations, this study shifts focus toward a modeling paradigm that emphasizes structural transparency, aligning more closely with the intrinsic characteristics of medical data. We propose a novel method, Channel Imposed Fusion (CIF), which enhances the signal-to-noise ratio through cross-channel information fusion, effectively reduces redundancy, and improves classification performance. Furthermore, we integrate CIF with the Temporal Convolutional Network (TCN), known for its structural simplicity and controllable receptive field, to construct an efficient and explicit classification framework. Experimental results on multiple publicly available EEG and ECG datasets demonstrate that the proposed method not only outperforms existing state-of-the-art (SOTA) approaches in terms of various classification metrics, but also significantly enhances the transparency of the classification process, offering a novel perspective for medical time series classification.

==> TEX/Conclusion.tex <==
\section{Conclusion}
In this paper, we propose a simple yet effective temporal classification representation method called Channel-Imposed Fusion (CIF) and combine it with a straightforward TCN structure. This approach outperforms current SOTA methods on multiple medical time-series datasets. Additionally, the CIF method demonstrates strong adaptability, enabling integration with cutting-edge methods to further enhance their performance. \textbf{Through the CIF method, we aim to show researchers in the field that, rather than solely modifying models to process high-level features, exploring the underlying core features of the data itself is also a research path worth delving into.}

==> TEX/lim.tex <==
\section{Limitations}
Biomedical time series exhibit complex modal characteristics, which lead to significant efficiency bottlenecks when manually adjusting the prior parameters (t, n, a, b) with clear medical interpretations in the CIF model based on empirical experience. This limitation highlights the urgent need for developing novel automated hyperparameter optimization frameworks.

==> TEX/process_data.tex <==

\begin{table}[!htbp]
    \centering
    \scriptsize
    \caption{\textbf{The information of processed datasets.} The table shows the number of subjects, samples, classes, channels, sampling rate, sample timestamps, modality of MedTS, and file size. Here, \textbf{\#-Timestamps} indicates the number of timestamps per sample.All data processing procedures follow those of Medformer~\cite{wang2024medformer}.
    }
    % \vspace{-3mm}
    \label{tab:processed_data}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}ll|cccccccc@{}}
    \toprule
    \multicolumn{2}{l|}{Datasets} & \#-Subject & \#-Sample & \#-Class & \#-Channel & \#-Timestamps & Sampling Rate & Modality & File Size  \\ \midrule
    \multicolumn{2}{l|}{APAVA} &  23     & 5,967 &  2  & 16 & 256 &  256Hz  & EEG & 186MB \\
    \multicolumn{2}{l|}{ADFTD} &  88  & 69,752 &  3  & 19 & 256 &  256Hz  & EEG & 2.52GB \\
    \multicolumn{2}{l|}{TDBrain} &  72  & 6,240 &  2  & 33 & 256 &  256Hz  & EEG & 571MB \\
    \multicolumn{2}{l|}{PTB} &  198  & 64,356 &  2  & 15 & 300 &  250Hz  & ECG & 2.15GB \\
    \multicolumn{2}{l|}{PTB-XL} &  17,596  & 191,400 &  5  & 12 & 250 &  250Hz  & ECG & 4.28GB \\
    % \multicolumn{2}{l|}{EEGMMIDB} &  106  & 9236 &  3  & 64 & 640 &  160Hz  & Type-II & 2.82GB \\
    % \multicolumn{2}{l|}{WG-fNIRS} &  26  & 9360 &  2  & 72 & 25 &  10Hz  & Type-II & 129MB \\
    \bottomrule
    \end{tabular}
    } % End of first resizebox
    % \vspace{-8mm}
\end{table}


\begin{table}[thbp]
    \centering
    \caption{Datasets and mapping details of UEA dataset \citep{bagnall2018uea}.}
      \vskip 0.1in
    \label{tab:uea_datasets}
    \begin{tabular}{|l|c c | c | c|}
        \hline
        Dataset & Sample Numbers(train set,test set) & Variable Number & Series Length \\
        \hline
        EthanolConcentration & (261, 263) & 3 & 1751 \\
        FaceDetection & (5890, 3524) & 144 & 62 \\
        Handwriting & (150, 850) & 3 & 152 \\
        Heartbeat & (204, 205) & 61 & 405 \\
        JapaneseVowels & (270, 370) & 12 & 29 \\
        PEMSSF & (267, 173) & 963 & 144 \\
        SelfRegulationSCP1 & (268, 293) & 6 & 896 \\
        SelfRegulationSCP2 & (200, 180) & 7 & 1152 \\
        SpokenArabicDigits & (6599, 2199) & 13 & 93 \\
        UWaveGestureLibrary & (120, 320) & 3 & 315 \\
        \hline
    \end{tabular}
\end{table}

==> Tab/tab_sub_ind.tex <==

\begin{table}
\centering
% \scriptsize
\def\arraystretch{0.95}
\caption{\textbf{Results of Subject-Independent Setup.} 
% Results of the APAVA, TDBrain, ADFTD, PTB, and PTB-XL datasets under this setup are presented here.
The results we compare include those reported by Medforme~\cite{wang2024medformer} and MedGNN~\cite{fan2025medgnn}. Additionally, we have reproduced all the methods in the Table \ref{tab:subject-independent-reproduce} to ensure a \textbf{fairer comparison}.The best result is highlighted in \textbf{bold}, and the second-best is \underline{underlined}.
}
\label{tab:subject-independent-report}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    % \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy \uparrow}} & \multicolumn{1}{c}{\textbf{Precision \uparrow}} & \multicolumn{1}{c}{\textbf{Recall \uparrow}} & \multicolumn{1}{c}{\textbf{F1 score \uparrow}} & \multicolumn{1}{c}{\textbf{AUROC \uparrow}} & \multicolumn{1}{c}{\textbf{AUPRC \uparrow}}  \\
      \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy $\uparrow$}} & \multicolumn{1}{c}{\textbf{Precision $\uparrow$}} & \multicolumn{1}{c}{\textbf{Recall $\uparrow$}} & \multicolumn{1}{c}{\textbf{F1 score $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUROC $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUPRC $\uparrow$}} \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{APAVA} \\ (2-Classes) \\Reported} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} &    68.64\std{1.82} & 68.48\std{2.10} & 68.77\std{2.27} & 68.06\std{1.94} & 75.94\std{3.61} & 74.38\std{4.05} \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 73.77\std{1.95} & 79.29\std{4.36} & 68.86\std{1.70} & 68.93\std{1.85} & 72.39\std{3.33} & 72.05\std{3.65} \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 74.94\std{2.15} & 74.59\std{1.50} & 73.56\std{3.55} & 73.51\std{3.39} & 83.72\std{1.97} & 82.94\std{2.37}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 73.11\std{4.40} & 75.17\std{6.06} & 69.17\std{4.56} & 69.47\std{5.06} & 70.46\std{4.91} & 70.75\std{5.27}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 74.55\std{1.66} & 74.77\std{2.10} & 71.76\std{1.72} & 72.30\std{1.79} & 85.59\std{1.55} & \underline{84.39\std{1.57}} \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 71.14\std{1.59} & 79.30\std{0.97} & 65.27\std{2.28} & 64.01\std{3.16} & 68.87\std{2.34} & 71.06\std{1.60} \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 71.89\std{3.81} & 71.80\std{4.58} & 69.44\std{3.56} & 69.74\std{3.84} & 70.55\std{2.96} & 70.78\std{4.08}  \\
    & \textbf{PatchTST}~\cite{nie2022time}   & 67.03\std{1.65} & 78.76\std{1.28} & 59.91\std{2.02} & 55.97\std{3.10} & 65.65\std{0.28} & 67.99\std{0.76}  \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 78.70\std{2.00} & 82.50\std{3.95} & 75.00\std{1.61} & 75.93\std{1.82} & 73.94\std{1.40} & 76.04\std{1.14}  \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 76.30\std{4.72} & 77.64\std{5.95} & 73.09\std{5.01} & 73.75\std{5.38} & 72.50\std{6.60} & 73.23\std{7.60} \\
    % & \textbf{Medformer}  & 78.74\std{0.64} & 81.11\std{0.84} & 75.40\std{0.66} & 76.31\std{0.71} & 83.20\std{0.91} & 83.66\std{0.92} & 36s\std{0.00} \\
    & \textbf{Medformer}~\cite{wang2024medformer} & 78.74\std{0.64} & 81.11\std{0.84} & 75.40\std{0.66} & 76.31\std{0.71} & 83.20\std{0.91} & 83.66\std{0.92} \\
  
     & \textbf{MedGNN}~\cite{fan2025medgnn} & \underline{82.60\std{0.35}} & \textbf{87.70\std{0.22}} & \underline{78.93\std{0.09}} & \underline{80.25\std{0.16}} & \underline{85.93\std{0.26}} & - \\
     & \textbf{HM-BiTCN + CIF} & \textbf{85.16\std{1.55}} & \underline{84.76\std{1.62}} & \textbf{85.33\std{1.27}} & \textbf{84.82\std{1.49}} & \textbf{94.06\std{1.07}} & \textbf{94.21\std{0.99}}  \\

    % & \textbf{HM-BiTCN + CIC V2} & 87.37\std{1.48}& 89.11\std{1.13}& 85.35\std{1.99}& 86.36\std{1.78}& 96.37\std{0.92}& 96.35\std{0.90} \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{TDBrain} \\ (2-Classes) \\Reported} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 87.33\std{3.79} & 88.06\std{3.56} & 87.33\std{3.79} & 87.26\std{3.84} & 93.81\std{2.26} & 93.32\std{2.42}  \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 81.56\std{2.19} & 81.97\std{2.25} & 81.56\std{2.19} & 81.50\std{2.20} & 91.20\std{1.78} & 91.51\std{1.71}  \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 78.13\std{1.98} & 78.52\std{1.91} & 78.13\std{1.98} & 78.04\std{2.01} & 86.56\std{1.86} & 86.48\std{1.99}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 89.02\std{2.50} & 89.43\std{2.14} & 89.02\std{2.50} & 88.98\std{2.54} & 96.64\std{0.68} & \underline{96.75\std{0.63}}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 74.67\std{1.06} & 74.71\std{1.06} & 74.67\std{1.06} & 74.65\std{1.06} & 83.37\std{1.14} & 83.73\std{1.27}  \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 76.96\std{3.76} & 77.24\std{3.59} & 76.96\std{3.76} & 76.88\std{3.83} & 85.27\std{4.46} & 82.81\std{5.64}  \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 87.88\std{2.48} & 88.86\std{1.84} & 87.88\std{2.48} & 87.78\std{2.56} & 97.05\std{0.68} & 96.99\std{0.68} \\
    & \textbf{PatchTST}~\cite{nie2022time}   & 79.25\std{3.79} & 79.60\std{4.09} & 79.25\std{3.79} & 79.20\std{3.77} & 87.95\std{4.96} & 86.36\std{6.67} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 87.92\std{2.01} & 88.64\std{1.40} & 87.92\std{2.01} & 87.85\std{2.08} & 96.30\std{0.54} & 96.40\std{0.45}  \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 87.17\std{1.67} & 87.99\std{1.68} & 87.17\std{1.67} & 87.10\std{1.68} & 96.28\std{0.92} & 96.34\std{0.81}  \\
    & \textbf{Medformer }~\cite{wang2024medformer}  & 89.62\std{0.81} & 89.68\std{0.78} & 89.62\std{0.81} & 89.62\std{0.81} & 96.41\std{0.35} & 96.51\std{0.33}  \\
     & \textbf{MedGNN }~\cite{fan2025medgnn}  & \underline{91.04\std{0.09}} & \underline{91.15\std{0.12}} & \underline{91.04\std{0.20}} & \underline{91.04\std{0.08}} & \underline{96.74\std{0.04}} & - \\

     & \textbf{HM-BiTCN + CIF}  & \textbf{93.13\std{1.41}} & \textbf{93.33\std{1.37}} & \textbf{93.13\std{1.41}} & \textbf{93.12\std{1.42}} & \textbf{98.62\std{0.66}} & \textbf{98.68\std{0.63}}\\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{ADFTD} \\ (3-Classes) \\Reported} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 45.25\std{1.48} & 43.67\std{1.94} & 42.96\std{2.03} & 42.59\std{1.85} & 61.02\std{1.82} & 43.10\std{2.30}  \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 50.45\std{2.31} & 45.57\std{1.63} & 45.88\std{1.82} & 45.50\std{1.70} & 66.45\std{2.03} & 48.33\std{2.05}  \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 46.30\std{0.59} & 46.05\std{0.76} & 44.22\std{1.38} & 43.91\std{1.37} & 62.62\std{1.75} & 46.11\std{1.44}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 48.45\std{1.96} & 46.54\std{1.68} & 46.06\std{1.84} & 45.74\std{1.38} & 65.87\std{1.27} & 47.60\std{1.30}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 52.60\std{1.59} & 46.79\std{1.27} & 47.28\std{1.29} & 46.79\std{1.13} & 67.26\std{1.16} & 49.53\std{1.21} \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 45.60\std{2.03} & 44.70\std{1.33} & 45.05\std{1.30} & 44.31\std{1.74} & 62.50\std{0.81} & 45.16\std{0.85}  \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 49.95\std{1.05} & 47.71\std{0.97} & 47.46\std{1.50} & 46.96\std{1.35} & 66.23\std{1.37} & 47.33\std{1.78}  \\
    & \textbf{PatchTST}~\cite{nie2022time}   & 44.37\std{0.95} & 42.40\std{1.13} & 42.06\std{1.48} & 41.97\std{1.37} & 60.08\std{1.50} & 42.49\std{1.79}  \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 50.78\std{1.17} & 49.64\std{1.49} & 49.89\std{1.67} & 47.94\std{0.69} & 69.17\std{1.58} & \underline{51.73\std{1.94}} \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 50.47\std{2.14} & 49.13\std{1.83} & 48.01\std{1.53} & 48.09\std{1.59} & 67.93\std{1.59} & 48.93\std{2.02} \\
    & \textbf{Medformer }~\cite{wang2024medformer}  & 53.27\std{1.54} & 51.02\std{1.57} & 50.71\std{1.55} & 50.65\std{1.51} & 70.93\std{1.19} & 51.21\std{1.32} \\
    & \textbf{MedGNN }~\cite{fan2025medgnn}  & \underline{56.12\std{0.11}} & \underline{55.07\std{0.09}} & \underline{55.47\std{0.34}} & \underline{55.00\std{0.24}} & \underline{74.68\std{0.33}} & -   \\
      & \textbf{HM-BiTCN + CIF}  & \textbf{58.56\std{0.93}} & \textbf{55.65\std{0.81}} & \textbf{55.86\std{0.79}} & \textbf{55.42\std{0.82}} & \textbf{76.07\std{0.59}} & \textbf{59.75\std{0.67}} \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB} \\ (2-Classes) \\ Reported} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 73.35\std{2.10} & 72.11\std{2.89} & 63.24\std{3.17} & 63.69\std{3.84} & 78.54\std{3.48} & 74.25\std{3.53}  \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 80.17\std{3.79} & 85.04\std{1.83} & 71.25\std{6.29} & 72.75\std{7.19} & 88.55\std{3.45} & 87.31\std{3.25}  \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 76.05\std{2.54} & 77.58\std{3.61} & 66.10\std{3.55} & 67.14\std{4.37} & 85.93\std{4.31} & 82.59\std{5.42}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 78.69\std{1.68} & 82.87\std{1.02} & 69.19\std{2.90} & 70.84\std{3.47} & 92.09\std{0.53} & 90.02\std{0.60}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 83.89\std{0.71} & \underline{88.25\std{1.18}} & 76.39\std{1.01} & 79.06\std{1.06} & 91.18\std{1.16} & \underline{90.93\std{0.98}}  \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 76.59\std{1.90} & 79.88\std{1.90} & 66.31\std{2.95} & 67.38\std{3.71} & 86.86\std{2.75} & 83.75\std{2.84}  \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 78.66\std{0.49} & 82.77\std{0.86} & 69.12\std{0.87} & 70.90\std{1.00} & 89.37\std{2.51} & 86.67\std{2.38}  \\
    & \textbf{PatchTST}~\cite{nie2022time}   & 74.74\std{1.62} & 76.94\std{1.51} & 63.89\std{2.71} & 64.36\std{3.38} & 88.79\std{0.91} & 83.39\std{0.96} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 77.96\std{2.13} & 81.72\std{1.61} & 68.20\std{3.35} & 69.65\std{3.88} & 91.13\std{0.74} & 88.42\std{1.30} \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 77.37\std{1.02} & 81.84\std{0.66} & 67.14\std{1.80} & 68.47\std{2.19} & 90.08\std{1.76} & 87.22\std{1.68}  \\
    & \textbf{Medformer }~\cite{wang2024medformer}  & 83.50\std{2.01} & 85.19\std{0.94} & 77.11\std{3.39} & 79.18\std{3.31} & 92.81\std{1.48} & 90.32\std{1.54}  \\
     & \textbf{MedGNN }~\cite{fan2025medgnn}  & \underline{84.53\std{0.28}} & 87.35\std{0.45} & \underline{77.90\std{0.66}} & \underline{80.40\std{0.62}} & \underline{93.31\std{0.46}} & - \\

     & \textbf{HM-BiTCN + CIF}  & \textbf{88.29\std{1.45}} & \textbf{90.66\std{1.48}} & \textbf{83.21\std{2.02}} & \textbf{85.59\std{1.96}} & \textbf{94.28\std{0.93}} & \textbf{93.78\std{1.11}}  \\

     
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB-XL} \\ (5-Classes) \\ Reported} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 61.68\std{2.72} & 51.60\std{1.64} & 49.10\std{1.52} & 48.85\std{2.27} & 82.04\std{1.44} & 51.93\std{1.71}  \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 73.30\std{0.14} & 65.06\std{0.35} & \textbf{61.23\std{0.33}} & \underline{62.59\std{0.14}} & 90.02\std{0.06} & \underline{67.43\std{0.22}} \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 57.20\std{9.47} & 52.38\std{6.09} & 49.04\std{7.26} & 47.89\std{8.44} & 82.13\std{4.17} & 52.31\std{7.03}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 71.43\std{0.32} & 62.64\std{0.60} & 59.12\std{0.47} & 60.44\std{0.43} & 88.65\std{0.09} & 64.76\std{0.17}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 69.28\std{0.22} & 59.59\std{0.45} & 54.62\std{0.18} & 56.20\std{0.19} & 86.71\std{0.10} & 60.27\std{0.21}  \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 72.14\std{0.27} & 63.84\std{0.72} & 60.01\std{0.81} & 61.43\std{0.38} & 88.97\std{0.33} & 65.83\std{0.51}   \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 70.56\std{0.55} & 61.57\std{0.66} & 57.75\std{0.72} & 59.10\std{0.66} & 88.32\std{0.36} & 63.40\std{0.79} \\
    & \textbf{PatchTST}~\cite{nie2022time}   & 73.23\std{0.25} & \underline{65.70\std{0.64}} & 60.82\std{0.76} & \textbf{62.61\std{0.34}} & 89.74\std{0.19} & 67.32\std{0.22} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 71.72\std{0.43} & 63.12\std{1.02} & 59.20\std{0.75} & 60.69\std{0.18} & 88.80\std{0.24} & 64.72\std{0.47}  \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 70.59\std{0.44} & 61.57\std{0.65} & 57.62\std{0.35} & 59.05\std{0.25} & 88.21\std{0.16} & 63.36\std{0.29}  \\
    & \textbf{Medformer }~\cite{wang2024medformer} & 72.87\std{0.23} & 64.14\std{0.42} & 60.60\std{0.46} & 62.02\std{0.37} & 89.66\std{0.13} & 66.39\std{0.22}  \\
    & \textbf{MedGNN}~\cite{fan2025medgnn} & \textbf{73.87\std{0.18}} & \textbf{66.26\std{0.29}} & \underline{61.13\std{0.29}} & 62.54\std{0.20} & \underline{90.21\std{0.15}} & - \\
    %  & \textbf{HM-BiTCN + CIF}  & 73.32\std{1.06} & 64.81\std{1.93} & 61.12\std{0.60} & 62.01\std{0.84} & \textbf{90.25\std{0.75}} & 67.31\std{1.55}  \\
      & \textbf{HM-BiTCN + CIF}  & \underline{73.73\std{0.30}}& 65.41\std{0.67}& 60.70\std{1.08}& 61.89\std{0.91}& \textbf{90.53\std{0.22}}& \textbf{67.75\std{0.75}}\\
      
    \bottomrule
\end{tabular}
}
\end{table}

\subsection{Results of Subject-Dependent}

\subsubsection{Efficiency Analysis}
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
       \includegraphics[width=\linewidth]{pic/qipao_APAVA.pdf}
        \caption{APAVA-Subject}  % 自动显示 (a)
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
          \includegraphics[width=\linewidth]{pic/qipao_TDBrain.pdf}
        \caption{TDBRAIN-Subject}  % 自动显示 (b)
    \end{subfigure}
    \caption{Model effectiveness and efficiency comparison on
two datasets under the Subject-based setup.} 
        \label{fig_APAVA_TDBrain}
\end{figure}
We evaluate the model efficiency in terms of accuracy, training speed, and memory footprint using two datasets: APAVA and TDBRAIN. In Figure~\ref{fig_APAVA_TDBrain}, a marker closer to the upper-left corner indicates higher accuracy and faster training speed, while a smaller marker area corresponds to lower memory usage. The results show that HM-BiTCN achieves the best overall performance among all baseline methods, demonstrating its high efficiency and reliability across different application scenarios.

==> sections/Ablation.tex <==

% To thoroughly evaluate the effectiveness and generalizability of the proposed method, we conduct the following three ablation studies:

% \textbf{(1) Effectiveness of CIF Method Integration:} We incorporate the proposed Channel-Imposed Fusion (CIF) theory into the HM-BiTCN architecture to evaluate its contribution to performance. This experiment aims to verify whether explicitly modeling inter-channel causal dependencies can enhance the model's ability to capture pathological patterns in medical time-series data. More details can be found in Appendix \ref{app:module_study_CIC}.
\textbf{(1) Effectiveness of CIF:} Table \ref{tab:abl_differential} demonstrates the excellent performance of combining HM-BiTCN with CIF, confirming the compatibility of the HM-BiTCN with CIF. See Appendix~\ref{app:module_study_CIC} for details.
% We integrate the proposed Channel-Imposed Fusion (CIF) into HM-BiTCN to evaluate its impact on capturing inter-channel dependencies and improving performance. See Appendix~\ref{app:module_study_CIC} for details.
\begin{table}[!h]
    \centering
    \caption{Exploring the Integration of HM-BiTCN Structure with CIF.}
    \label{tab:abl_differential}
    \scalebox{0.8}{
    \begin{tabular}{l c | c c | c c | c c | c c}
        \toprule[1.5pt]
        \multicolumn{2}{c|}{Datasets} & \multicolumn{2}{c|}{APAVA} & \multicolumn{2}{c|}{ADFTD} & \multicolumn{2}{c|}{PTB} & \multicolumn{2}{c}{TDBRAIN} \\
        \cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}
        \multicolumn{2}{c|}{Metrics} & Accuracy & F1 Score & Accuracy & F1 Score & Accuracy & F1 Score & Accuracy & F1 Score\\
        \midrule[1pt]
        \multicolumn{2}{c|}{w/ CIF}   & 85.16\std{1.55} & 84.82\std{1.49} & 58.56\std{0.93} & 55.42\std{0.82} & 88.29\std{1.45} & 85.59\std{1.96} & 93.13\std{1.41} & 93.12\std{1.42}  \\
        \multicolumn{2}{c|}{w/o CIF} & 82.49\std{1.40} & 81.60\std{1.39} & 52.05\std{2.22} & 49.48\std{2.70} & 81.87\std{1.87} & 75.84\std{3.20}  & 84.90\std{2.60} & 84.76\std{2.74}\\
        \midrule[1pt]
        \multicolumn{2}{c|}{\textcolor{blue}{\textbf{Improvement}}} 
            & \textcolor{blue}{\textbf{+2.67\%}} & \textcolor{blue}{\textbf{+3.22\%}} 
            & \textcolor{blue}{\textbf{+6.51\%}} & \textcolor{blue}{\textbf{+5.94\%}} 
            & \textcolor{blue}{\textbf{+6.42\%}} & \textcolor{blue}{\textbf{+9.75\%}}
            & \textcolor{blue}{\textbf{+8.23\%}} & \textcolor{blue}{\textbf{+8.36\%}} \\
        \bottomrule[1.5pt]
    \end{tabular}
    }
\end{table}
    
%  \textbf{(2) Generalizability of Hyperparameters:} We transfer the key hyperparameters obtained from HM-BiTCN—such as the fusion coefficients ($a$, $b$), and segment length ($n$)—to other baseline models. This experiment evaluates whether these hyperparameters retain effectiveness when applied to different architectures, indicating their robustness and broader applicability. More details can be found in Appendix \ref{app:Generalizability of Hyperparameters}.
    
% \textbf{(3) Fine-tuning Transferred Parameters:} For models where the transferred hyperparameters from HM-BiTCN do not yield optimal results, we perform additional fine-tuning. More details can be found in Appendix \ref{app:Fine-tuning Transferred Parameters:}. Figure \ref{fig_APAVA_TDBrain_PTB_APAVA} shows the effect of combining CIF with other methods.

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%        \includegraphics[width=\linewidth]{pic/APAVA+CIF.pdf}
%         \caption{APAVA}  % 自动显示 (a)
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/TDBrain+CIF.pdf}
%         \caption{TDBRAIN}  % 自动显示 (b)
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/PTB+CIF.pdf}
%         \caption{PTB}  % 自动显示 (b)ADFTD
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/ADFTD+CIF.pdf}
%         \caption{ADFTD}  % 自动显示 (b)
%     \end{subfigure}
%     \caption{The improvements achieved by various baselines when combined with the CIF method.} 
%         \label{fig_APAVA_TDBrain_PTB_APAVA}
% \end{figure}

\textbf{(2) Hyperparameter Transfer and Adaptation:} We evaluate the transferability of key hyperparameters (e.g., $a$, $b$, $n$) from HM-BiTCN to other models. If transferred settings underperform, we further fine-tune them for adaptation. See Appendices~\ref{app:Generalizability of Hyperparameters} and~\ref{app:Fine-tuning Transferred Parameters}.
Figure \ref{fig_APAVA_TDBrain_PTB_APAVA} illustrates the outstanding performance of CIF when combined with other models. 
% The integration process involves two steps. First, we conduct hyperparameter transfer by applying CIF-based parameters to the HM-BiTCN model. Second, for the few cases where no improvement is observed after hyperparameter transfer, we perform additional fine-tuning to optimize the results.
\begin{figure}[ht]
    \centering

    \begin{subfigure}{0.48\textwidth}
        \centering
          \includegraphics[width=\linewidth]{pic/_TDBrain.pdf}
        \caption{TDBRAIN}  % 自动显示 (b)
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
          \includegraphics[width=\linewidth]{pic/_PTB.pdf}
        \caption{PTB}  % 自动显示 (b)ADFTD
    \end{subfigure}
    \hfill
    % \begin{subfigure}{0.48\textwidth}
    %     \centering
    %       \includegraphics[width=\linewidth]{pic/ADFTD+CIF.pdf}
    %     \caption{ADFTD}  % 自动显示 (b)
    % \end{subfigure}
    \caption{The improvements achieved by various baselines when combined with the CIF method.} 
        \label{fig_APAVA_TDBrain_PTB_APAVA}
\end{figure}
% \begin{itemize}
% \item \textbf{Effectiveness of CIC Theory Integration:} We incorporate the proposed Channel-Imposed Causality (CIC) theory into the HM-BiTCN architecture to evaluate its contribution to performance. This experiment aims to verify whether explicitly modeling inter-channel causal dependencies can enhance the model's ability to capture pathological patterns in medical time-series data. More details can be found in Appendix \ref{app:ablation_study}.
    
% \item \textbf{Generalizability of Hyperparameters:} We transfer the key hyperparameters obtained from HM-BiTCN—such as the fusion coefficients ($a$, $b$), and segment length ($n$)—to other baseline models. This experiment evaluates whether these hyperparameters retain effectiveness when applied to different architectures, indicating their robustness and broader applicability. More details can be found in Appendix \ref{app:Generalizability of Hyperparameters}.
    
% \item \textbf{Fine-tuning Transferred Parameters:} For models where the transferred hyperparameters from HM-BiTCN do not yield optimal results, we perform additional fine-tuning. This step investigates the adaptability of CIC-related parameters and explores how they can be optimized for other model structures. More details can be found in Appendix \ref{app:Fine-tuning Transferred Parameters:}.
% \end{itemize}

==> sections/Broader_Impacts.tex <==
In this study, we take the first step toward a paradigm shift in medical time-series analysis, transitioning from a focus on model architecture improvements to emphasizing the intrinsic structure of the data. Our experimental results, which outperform several state-of-the-art methods across multiple datasets, validate the effectiveness of this approach. We emphasize that uncovering the essential characteristics in medical time-series data is a valuable research direction, particularly given the critical need for model interpretability in medical applications. However, practitioners should be cognizant of the method’s limitations.



==> sections/Conclusion.tex <==

% \textbf{Conclusion}  
In this paper, we propose a simple yet effective temporal classification representation method called Channel-Imposed Fusion (CIF) and combine it with a straightforward TCN structure. This approach outperforms current SOTA methods on multiple medical time-series datasets. Additionally, the CIF method demonstrates strong adaptability, enabling integration with cutting-edge methods to further enhance their performance. \textbf{Through the CIF method, we aim to show researchers in the field that, rather than solely modifying models to process high-level features, exploring the underlying core features of the data itself is also a research path worth delving into.}

% \textbf{Limitations and Future Work}
% Our HM-BiTCN structure is relatively simple and still somewhat crude. We believe that future work can focus on designing a structure better suited to the CIC theory. Additionally, we plan to explore a more universal paradigm for time-series analysis in our future research.

==> sections/EXPset.tex <==

% We compared our method with 12 baseline methods across 5 datasets, including 3 EEG datasets and 2 ECG datasets. The evaluation was conducted under two setups (Section~\ref{sec:preliminary}): subject-dependent and subject-independent. In the subject-dependent setup, the training, validation, and test sets were split based on samples; while in the subject-independent setup, the data were split based on different subjects. In the subject-dependent setup, we combined the \textit{Channel-Imposed Fusion} method with the Medformer method to explore the application potential of this theory.
% \textbf{In the more challenging subject-independent setup}, we compared the proposed HM-BiTCN method with existing methods and achieved encouraging results. This experiment not only helped us evaluate the performance of different methods under varying setups, but also revealed the potential for performance improvement by integrating advanced theoretical insights.


\textbf{Datasets.}
(1) \textbf{\textsc{APAVA}}~\cite{escudero2006analysis} is an EEG dataset where each sample is assigned a binary label indicating whether the subject has Alzheimer’s disease. (2) \textbf{\textsc{TDBrain}}~\cite{van2022two} is an EEG dataset with a binary label assigned to each sample, indicating whether the subject has Parkinson’s disease. (3) \textbf{\textsc{ADFTD}}~\cite{miltiadous2023dataset,miltiadous2023dice} is an EEG dataset with a three-class label for each sample, categorizing the subject as Healthy, having Frontotemporal Dementia, or Alzheimer’s disease. (4) \textbf{\textsc{PTB}}~\cite{physiobank2000physionet} is an ECG dataset where each sample is labeled with a binary indicator of Myocardial Infarction. (5) \textbf{\textsc{PTB-XL}}~\cite{wagner2020ptb} is an ECG dataset with a five-class label for each sample, representing various heart conditions. Table~\ref{tab:processed_data} provides information on the processed datasets.The data processing methodology is the same as that of Medformer~\cite{wang2024medformer} and MedGNN~\cite{fan2025medgnn}.
% For additional details on data characteristics, train-validation-test splits under different setups, and data preprocessing, please see Appendix~\ref{app:data_preprocessing}.



\textbf{Baselines.}
We compare with 12 state-of-the-art time series transformer methods: Autoformer~\cite{wu2021autoformer}, Crossformer~\cite{zhang2022crossformer}, FEDformer~\cite{zhou2022fedformer}, Informer~\cite{zhou2021informer}, iTransformer~\cite{liu2023itransformer}, MTST~\cite{zhang2024multi}, Nonformer~\cite{liu2022non}, PatchTST~\cite{nie2022time}, Reformer~\cite{kitaev2019reformer}, vanilla Transformer~\cite{vaswani2017attention}, Medformer~\cite{wang2024medformer}, MedGNN~\cite{fan2025medgnn}.



\textbf{Implementation.}
We employ six evaluation metrics: accuracy, precision (macro-averaged), recall (macro-averaged), F1 score (macro-averaged), AUROC (macro-averaged), and AUPRC (macro-averaged). The training process is conducted with five random seeds (41-45) on fixed training, validation, and test sets to compute the mean and standard deviation of the models. All experiments were conducted using an NVIDIA RTX 3090 GPU and implemented with PyTorch version 1.11.0~\cite{paszke2017automatic}.
% \input{table/subject_dependent}




==> sections/IMPLEMENTATION_DETAILS.tex <==
We implement our method and all the baselines based on the Time-Series-Library project\footnote{\url{https://github.com/thuml/Time-Series-Library}} from Tsinghua University~\cite{wu2023timesnet}, which integrates all methods under the same framework and training techniques to ensure a relatively fair comparison. The 12 baseline time series transformer methods are Autoformer~\cite{wu2021autoformer}, Crossformer~\cite{zhang2022crossformer}, FEDformer~\cite{zhou2022fedformer}, Informer~\cite{zhou2021informer}, iTransformer~\cite{liu2023itransformer}, MTST~\cite{zhang2024multi}, Nonformer~\cite{liu2022non}, PatchTST~\cite{nie2022time}, Reformer~\cite{kitaev2019reformer}, vanilla Transformer~\cite{vaswani2017attention}, Medformer~\cite{wang2024medformer}, and MedGNN~\cite{fan2025medgnn}.


\textbf{Autoformer}
Autoformer~\cite{wu2021autoformer} employs an auto-correlation mechanism to replace self-attention for time series forecasting. Additionally, they use a time series decomposition block to separate the time series into trend-cyclical and seasonal components for improved learning. The raw source code is available at \url{https://github.com/thuml/Autoformer}.

\textbf{Crossformer}
Crossformer~\cite{zhang2022crossformer} designs a single-channel patching approach for token embedding. They utilize two-stage self-attention to leverage both temporal features and channel correlations. A router mechanism is proposed to reduce time and space complexity during the cross-dimension stage. The raw code is available at \url{https://github.com/Thinklab-SJTU/Crossformer}.

\textbf{FEDformer}
FEDformer~\cite{zhou2022fedformer} leverages frequency domain information using the Fourier transform. They introduce frequency-enhanced blocks and frequency-enhanced attention, which are computed in the frequency domain. A novel time series decomposition method replaces the layer norm module in the transformer architecture to improve learning. The raw code is available at \url{https://github.com/MAZiqing/FEDformer}.

\textbf{Informer}
Informer~\cite{zhou2021informer} is the first paper to employ a one-forward procedure instead of an autoregressive method in time series forecasting tasks. They introduce ProbSparse self-attention to reduce complexity and memory usage. The raw code is available at \url{https://github.com/zhouhaoyi/Informer2020}.

\textbf{iTransformer}
iTransformer~\cite{liu2023itransformer} questions the conventional approach of embedding attention tokens in time series forecasting tasks and proposes an inverted approach by embedding the whole series of channels into a token. They also invert the dimension of other transformer modules, such as the layer norm and feed-forward networks. The raw code is available at \url{https://github.com/thuml/iTransformer}.

\textbf{MTST}
MTST~\cite{zhang2024multi} uses the same token embedding method as Crossformer and PatchTST. It highlights the importance of different patching lengths in forecasting tasks and designs a method that can take different sizes of patch tokens as input simultaneously. The raw code is available at \url{https://github.com/networkslab/MTST}.

\textbf{Nonformer}
Nonformer~\cite{liu2022non} analyzes the impact of non-stationarity in time series forecasting tasks and its significant effect on results. They design a de-stationary attention module and incorporate normalization and denormalization steps before and after training to alleviate the over-stationarization problem. The raw code is available at \url{https://github.com/thuml/Nonstationary_Transformers}.

\textbf{PatchTST}
PatchTST~\cite{nie2022time} embeds a sequence of single-channel timestamps as a patch token to replace the attention token used in the vanilla transformer. This approach enlarges the receptive field and enhances forecasting ability. The raw code is available at \url{https://github.com/yuqinie98/PatchTST}.

\textbf{Reformer}
Reformer~\cite{kitaev2019reformer} replaces dot-product attention with locality-sensitive hashing. They also use a reversible residual layer instead of standard residuals. The raw code is available at \url{https://github.com/lucidrains/reformer-pytorch}.

\textbf{Transformer}
Transformer~\cite{vaswani2017attention}, commonly known as the vanilla transformer, is introduced in the well-known paper "Attention is All You Need." It can also be applied to time series by embedding each timestamp of all channels as an attention token. The PyTorch version of the code is available at \url{https://github.com/jadore801120/attention-is-all-you-need-pytorch}.

\textbf{Medformer}
Medformer~\cite{wang2024medformer} uses cross-channel patch embedding to model spatiotemporal dependencies.The raw code is available at  \url{https://github.com/DL4mHealth/Medformer}

\textbf{MedGNN}
MedGNN~\cite{fan2025medgnn} employs multi-resolution spatiotemporal graph learning to extract dynamic features across multiple time scales.
The raw code is available at  \url{https://github.com/aikunyi/MedGNN}.

==> sections/abstract.tex <==

% Automated classification of medical time-series signals, such as EEG and ECG, is crucial for clinical decision support and early disease detection. However, current mainstream methods, especially Transformer-based architectures, rely heavily on complex models to capture relationships between time points through attention mechanisms. While these methods are powerful, the relationships they build are implicit, often difficult to interpret, and fail to fully consider the unique characteristics of medical time-series data. We propose the Channel Information Coupling (CIC) method, which emphasizes the inherent causal relationships between channels in medical time-series data. By explicitly embedding these causal relationships, such as physiological conduction delays in ECG signals or interactions between brain regions in EEG data, we provide a more interpretable approach. By combining CIC theory with a simple yet effective Temporal Convolutional Network (TCN) for classification, our method performs excellently across several public datasets, significantly outperforming current state-of-the-art Transformer models. This approach not only improves classification accuracy but also provides a clearer, more interpretable model for medical time-series analysis.

% The automated classification of medical time-series signals, such as EEG and ECG, is crucial for clinical decision support and early disease detection. However, current mainstream methods, particularly Transformer-based architectures, often rely on complex models to capture relationships between time points using attention mechanisms. While these methods are powerful, the relationships they model are implicit, often difficult to interpret, and fail to fully account for the unique characteristics of medical time-series data. We propose the Channel-Imposed Fusion (CIF) method, which emphasizes the inherent temporal delays between channels in medical time-series data. By explicitly modeling these delays, such as physiological conduction delays in ECG signals or interactions between different brain regions in EEG data, we provide a more interpretable approach. By combining CIF method with a simple yet effective Temporal Convolutional Network (TCN) for classification, our method performs excellently across several public datasets, significantly outperforming current state-of-the-art(SOTA) Transformer models. This approach not only improves classification accuracy but also offers a clearer and more interpretable model for medical time-series analysis.

% The automatic classification of medical time-series signals, such as electroencephalography (EEG) and electrocardiography (ECG), plays a vital role in clinical decision support and early disease detection. While current mainstream approaches—particularly Transformer-based models—have demonstrated strong modeling capabilities by implicitly capturing temporal dependencies through attention mechanisms, they often rely on complex architectures. Moreover, the learned relationships are typically difficult to interpret and fail to fully exploit the intrinsic properties of medical time-series data.
% To address these challenges, we propose a novel method called \textit{Channel-Imposed Fusion} (CIF), which explicitly models the temporal relationships across different channels. This approach effectively reduces the high redundancy commonly found in EEG and ECG signals while enhancing the diversity of extracted features, thereby improving interpretability. We integrate CIF with a Temporal Convolutional Network (TCN), a model known for its simplicity and strong performance, to construct an efficient classification framework.
% Extensive experiments on multiple publicly available medical time-series datasets demonstrate that our method significantly outperforms state-of-the-art(SOTA) Transformer-based models in classification accuracy. Furthermore, our approach offers a more transparent and interpretable modeling paradigm, providing a promising direction for medical time-series analysis in real-world clinical applications.

% Automatic classification of medical time series signals, such as electroencephalogram (EEG) and electrocardiogram (ECG), plays a pivotal role in clinical decision support and early disease screening. Although Transformer-based models have achieved notable performance by implicitly modeling temporal dependencies through self-attention mechanisms, their inherently complex architectures and opaque reasoning processes undermine their trustworthiness in high-stakes clinical settings. In response to these limitations, this study shifts focus toward a modeling paradigm that emphasizes interpretability and structural transparency, aligning more closely with the intrinsic characteristics of medical data. We propose a novel method—\textbf{Channel-Imposed Fusion (CIF)}, which explicitly models temporal relationships across multiple channels, effectively reducing redundancy and enhancing feature diversity, thereby improving model interpretability. Furthermore, we integrate CIF with the Temporal Convolutional Network (TCN), known for its structural simplicity and controllable receptive field, to construct an efficient and interpretable classification framework. Experimental results on several public EEG and ECG datasets demonstrate that the proposed method not only surpasses current mainstream Transformer models in classification accuracy, but also achieves a desirable balance between performance and interpretability, thus offering a novel perspective for medical time series classification.
% We welcome all reviewers to reproduce our work.

The automatic classification of medical time series signals, such as electroencephalogram (EEG) and electrocardiogram (ECG), plays a pivotal role in clinical decision support and early detection of diseases. Although Transformer based models have achieved notable performance by implicitly modeling temporal dependencies through self-attention mechanisms, their inherently complex architectures and opaque reasoning processes undermine their trustworthiness in high stakes clinical settings. In response to these limitations, this study shifts focus toward a modeling paradigm that emphasizes structural transparency, aligning more closely with the intrinsic characteristics of medical data. 
We propose a novel method, \textbf{Channel Imposed Fusion (CIF)}, which enhances the signal‑to‑noise ratio through cross‑channel information fusion, effectively reduces redundancy, and improves classification performance.
% We propose a novel method \textbf{Channel Imposed Fusion (CIF)} that enhances the signal-to-noise ratio through cross-channel information fusion, effectively reducing redundancy and improving model classification capability. 
Furthermore, we integrate CIF with the Temporal Convolutional Network (TCN), known for its structural simplicity and controllable receptive field, to construct an efficient and explicit classification framework. 
% Experimental results on several public EEG and ECG datasets demonstrate that the proposed method not only surpasses the sota methods in classification accuracy but also achieves a desirable balance between performance and interpretability, thus offering a novel perspective for medical time series classification. 
Experimental results on multiple publicly available EEG and ECG datasets demonstrate that the proposed method not only outperforms existing state-of-the-art (SOTA) approaches in terms of various classification metrics, but also significantly enhances the transparency of the classification process, offering a novel perspective for medical time series classification.




==> sections/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \clearpage
% % \section*{NeurIPS Paper Checklist}
% \section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims made in abstract and introduction are supported by the results in Section~\ref{sec:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appendix~\ref{limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include theoretical results
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section~\ref{sec:experiments}, Appendix~\ref{app:reproduce_result} and Appendix~\ref{app:ablation_study}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include an anonymous link in the Abstract providing source codes with full implementation details for our methods and all baselines. All five datasets used for evaluation are publicly available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section~\ref{sec:experiments}, Appendix~\ref{app:data_preprocessing}, ~\ref{app:implementation_details},~\ref{app:reproduce_result} and \ref{app:ablation_study}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We run experiments over five random seeds and report the average value with the standard deviation. See Tables 1-3, 5-16.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Appendix~\ref{app:reproduce_result}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The authors follow the NeurIPS Code of Ethics during the conduct of this research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Section~\ref{Broader_Impacts} .
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not pose a high risk of misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We properly cite baseline models and the code library used for implementation. See Appendix~\ref{app:implementation_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not publish new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include crowdsourcing experiments nor research with
human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include crowdsourcing experiments nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The core methodological innovations of this paper do not involve large language models (LLMs).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/introduction.tex <==

Medical time series (MedTS) data, such as electroencephalogram (EEG) and electrocardiogram (ECG) signals, are widely used in clinical settings to monitor patient health and play a crucial role in diagnosing neurological and cardiovascular diseases~\cite{arif2024ef, xiao2023deep, zhu2025mtnet}. Accurate classification of these signals enables early anomaly detection, personalized treatment, and optimized therapy planning, ultimately improving patient outcomes and healthcare efficiency~\cite{liu2024classification, tian2023automatic}.
With advances in deep learning, CNN-based models like EEGNet \cite{lawhern2018eegnet} can automatically extract informative features from raw signals, significantly improving classification performance.

In recent years, Transformer models~\cite{vaswani2017attention}, powered by the self-attention mechanism~\cite{bahdanau2014neural}, have achieved remarkable progress in time-series modeling, particularly in capturing long-range dependencies and global contextual information~\cite{liu2021pyraformer, zhou2021informer}. By converting sequential data into high-dimensional token embeddings, Transformers are capable of modeling complex temporal dependencies implicitly. However, despite their strong performance across a range of time-series tasks, several limitations have emerged when applying Transformer-based architectures to medical time-series classification, particularly in the following aspects:
(1) Conflict Between Implicit Temporal Modeling and Explicit Physiological Mechanisms.
Conventional Transformer architectures employ self attention mechanisms to implicitly represent temporal dependencies . However, essential physiological dynamics in medical signals, including conduction delays between ECG leads and synchronization of EEG rhythms, require explicit structural representations. Although methods such as Medformer \cite{wang2024medformer} have adopted strategies involving multiple scales of embedding, their attention distributions still fail to directly correspond to the underlying biological processes. This leads to fundamental limitations in model interpretability.
(2) Mismatch Between Medical Domain Knowledge and Architectures Designed for General Purposes.
Mainstream time series modeling methods such as Autoformer~\cite{wu2021autoformer}, Informer~\cite{zhou2021informer}, and FEDformer~\cite{zhou2022fedformer} have achieved strong performance in general domains like weather forecasting and finance. However, their architectural designs fail to account for the unique structural characteristics of medical time series. Medical signals often exhibit high inter-channel redundancy, spatial dependencies among physiological leads, and distinct local morphological patterns. These important features are easily weakened or overlooked in the high-dimensional and implicit modeling processes of conventional Transformer architectures.




% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.5\textwidth}
%         \centering
%        \includegraphics[width=\linewidth]{pic/Implicit.pdf}
%         \caption{}  % 自动显示 (a)
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/Explicit.pdf}
%         \caption{}  % 自动显示 (b)
%     \end{subfigure}
%     \caption{(a) Implicitly construct the relationships between time series. (b) Explicitly construct the relationships between time series. The \textcolor{black}{$\leftrightarrow$} in different colors in the figure represent certain relationships.} 
%         \label{fig_Im_Ex}
% \end{figure}


\textbf{To address these limitations, we rethink the modeling paradigm from the perspective of data representation and break away from the conventional approach of implicitly discovering unknown temporal relationships. Unlike existing methods that rely on implicit learning, we advocate for explicitly modeling temporal relationships that have clear physical or physiological foundations. }
% \textbf{To address these limitations, we rethink the modeling paradigm by focusing on data representation and move beyond implicitly learning unknown temporal relationships. Instead, we explicitly model temporal dependencies grounded in clear physical or physiological principles.}
Based on this principle, we propose the \textit{Channel-Imposed Fusion} (CIF) method, which encodes prior causal structures directly into the feature representation. Specifically, CIF constructs new features through a linear combination of the form \( x_{\text{new}} = ax + by \), where \(x\) and \(y\) represent signals from two different channels, and \(a\) and \(b\) are predefined coefficients derived from domain knowledge. By embedding such structured prior knowledge into the model, CIF not only enhances the ability to capture critical pathological patterns but also significantly improves robustness and interpretability when dealing with noisy or irregular medical time-series data. This approach provides a more intuitive and effective framework for medical time-series analysis, contributing to the development of reliable clinical decision support systems.


Based on the design philosophy of the CIF method, we aim for the model to maintain high efficiency while ensuring good interpretability and simplifying the structure as much as possible. To this end, we propose a simple yet effective Hidden-layer Mixed Bidirectional Temporal Convolutional Network (HM-BiTCN) architecture. This architecture utilizes a hierarchical causal convolution module, which explicitly encodes the coupling relationships between channels and temporal dynamics, effectively avoiding the issues of poor interpretability and structural complexity caused by the implicit modeling of temporal dependencies in Transformer-based methods. 
Moreover, it is worth noting that the CIF method is not limited to the HM-BiTCN architecture; it has high portability and can be seamlessly integrated with existing Transformer architectures to enhance the model's adaptability and interpretability in medical time-series data.
\textbf{Our contributions are as follows:}

(1) \textbf{Proposing the Channel-Imposed Fusion (CIF) method}: We propose the CIF method to explicitly model the relationships between channel dimensions in medical time-series data, particularly for signals with clear physiological structures, such as EEG and ECG.
(2) \textbf{Designing the HM‑BiTCN model based on CIF}: We leverage the CIF method to construct the Hidden‑layer Mixed Bidirectional Temporal Convolutional Network (HM‑BiTCN), which explicitly models channel coupling and temporal dependencies. By adopting this TCN-based approach, HMBiTCN breaks the dominance of transformer models (SOTA) in MedTS classification and surpasses them across multiple datasets.
(3) \textbf{Providing methodological transferability}: 
The CIF method is not only applicable to the HM-BiTCN model but can also be seamlessly integrated into existing Transformer architectures. 
% \textbf{Our contributions are as follows:}
% \begin{itemize}
% \item \textbf{Channel-Imposed Fusion (CIF):} We propose CIF to explicitly model inter-channel temporal relationships in medical time-series data, especially those with clear physiological structures such as EEG and ECG.
% \item \textbf{HM-BiTCN architecture:} Based on CIF, we design the Hidden-layer Mixed Bidirectional Temporal Convolutional Network (HM-BiTCN), which captures both cross-channel coupling and temporal dependencies in an explicit and interpretable manner.
% \item \textbf{Beyond Transformer dominance:} Our TCN-based approach outperforms state-of-the-art Transformer models across multiple medical time-series classification benchmarks, challenging the current paradigm.
% \item \textbf{Transferable framework:} CIF is a flexible module that can be readily integrated into various neural architectures, including Transformer-based models, demonstrating strong theoretical and practical transferability.
% \end{itemize}



==> sections/method.tex <==



% In this section, we first introduce the CIC theory we propose and provide our explanation, followed by a description of the simple TCN structure we use.

\subsection{Channel-Imposed Fusion}
% \section{Data Fusion via Singular Value Decomposition}
\begin{figure}[htbp]
    \centering
 \includegraphics[
        width=\textwidth,
        height=0.7\textheight,  % 保持宽高比
        keepaspectratio,        % 防止变形
        ]{pic/CIF_t=1.pdf}
    % \includegraphics[scale=1.5]{your_pdf_file.pdf}
    \caption{The implementation process of the Channel-Imposed Fusion method.}
    \label{fig:your_label}
\end{figure}

In this section, we analyze the data fusion process using Singular Value Decomposition (SVD)~\cite{golub1971singular,klema1980singular}. Suppose the original time-series data matrix \( X \) has dimensions \( \mathbb{R}^{T \times C} \), where \( T \) represents the temporal length and \( C \) denotes the number of channels. We partition \( X \) along the channel dimension into two submatrices: the first \( n \) channels form \( X_{i} = X[:, :n] \), while the last \( n \) channels form \( X_{j} = X[:, -n:] \). The goal of fusion is to combine these two submatrices into a new representation:  
\begin{equation}
X_{fused} = a X_{i} + b X_{j},
\end{equation}
where \( a \) and \( b \) are learnable parameters that control the contribution of the front and back segments in the fused matrix. To understand this fusion process, we first apply SVD to both submatrices:
\begin{equation}
X_{i} = U_1 \Sigma_1 V_1^T, \quad X_{j} = U_2 \Sigma_2 V_2^T,
\end{equation}
where \( U_1, U_2 \in \mathbb{R}^{T \times T} \) are the left singular vectors representing temporal patterns, \( \Sigma_1, \Sigma_2 \in \mathbb{R}^{T \times n} \) are diagonal matrices containing the singular values that indicate the importance of each channel, and \( V_1, V_2 \in \mathbb{R}^{n \times n} \) are the right singular vectors capturing channel relationships. The fused matrix \( X_{\text{fused}} \) is then constructed by linearly combining these two matrices. Depending on the degree of similarity between \( X_{\text{i}} \) and \( X_{\text{j}} \), the fusion process either reduces redundancy or increases data diversity.  
When the correlation between \( X_{i} \) and \( X_{j} \) is high, their singular values and left singular vectors \( U_1 \) and \( U_2 \) are similar. This implies that both matrices capture similar temporal patterns, and the fused matrix \( X_{fused} \) primarily retains these common structures. Mathematically, if \( U_1 \approx U_2 \), the fused matrix can be approximated as:
\begin{equation}
X_{fused} \approx (a U_1 \Sigma_1 + b U_1 \Sigma_2) V_1^T.
\end{equation}
In this case, \( X_{fused} \) is largely determined by the shared temporal patterns \( U_1 \), while the weighted sum of \( \Sigma_1 \) and \( \Sigma_2 \) reflects the contribution of each channel. Since the temporal patterns are similar, the fusion process does not introduce significant new information, effectively reducing redundancy.  
On the other hand, when \( X_{i} \) and \( X_{j} \) have low correlation, their singular values and left singular vectors \( U_1 \) and \( U_2 \) differ significantly. This means that the two matrices capture distinct temporal patterns, and the fused matrix \( X_{fused} \) will combine these different components, enhancing data diversity. Mathematically, if \( U_1 \) and \( U_2 \) are dissimilar, the fused matrix can be expressed as:
\begin{equation}
X_{fused} = a U_1 \Sigma_1 V_1^T + b U_2 \Sigma_2 V_2^T.
\end{equation}

In this scenario, the fused matrix incorporates both the temporal patterns from \( U_1 \) and \( U_2 \), effectively combining the complementary information from both matrices. This leads to an increase in data diversity, as each matrix contributes distinct temporal patterns and channel relationships to the final fused representation. Thus, the fusion process allows for either redundancy reduction by preserving shared patterns or diversity enhancement by integrating complementary information, depending on the correlation between the front and back segments.

% In the two‐channel observation model \(x_1 = s_1 + \epsilon_1\) and \(x_2 = s_2 + \epsilon_2\), the signals and noises are zero-mean, mutually uncorrelated, stationary random processes with \(\mathrm{Var}(s_i) = \sigma_s^2\), \(\mathrm{Var}(\epsilon_i) = \sigma_\epsilon^2\), \(\mathrm{Cov}(s_1, s_2) = \rho\,\sigma_s^2\), and \(\mathrm{Cov}(\epsilon_1, \epsilon_2) = \gamma\,\sigma_\epsilon^2\), where typically \(\rho > \gamma\). The CIF produces an output \(y = a\,x_1 + b\,x_2\), whose signal-to-noise ratio (SNR) is given by \(\mathrm{SNR}_{\mathrm{out}} = \mathrm{SNR}_{\mathrm{in}} \cdot \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma}\). When \(ab < 0\), the numerator term \(2ab\,\rho\) becomes negative, helping to attenuate common-mode signal components, while the denominator term \(2ab\,\gamma\) also reduces noise cancellation, leading to \(\frac{a^2 + b^2}{(a + b)^2} > 1\), which suppresses shared interference. When \(ab > 0\) and \(\rho > \gamma\), signal components are reinforced more than noise, ensuring \(\mathrm{SNR}_{\mathrm{out}} > \mathrm{SNR}_{\mathrm{in}}\). This confirms that CIF is effective both in noise suppression and in signal enhancement.

% In the two‐channel observation model \(x_{front} = s_1 + \epsilon_1\) and \(x_{back} = s_2 + \epsilon_2\), the signals and noises are zero‐mean, mutually uncorrelated, stationary random processes with \(\mathrm{Var}(s_i) = \sigma_s^2\), \(\mathrm{Var}(\epsilon_i) = \sigma_\epsilon^2\), \(\mathrm{Cov}(s_1, s_2) = \rho\,\sigma_s^2\), and \(\mathrm{Cov}(\epsilon_1, \epsilon_2) = \gamma\,\sigma_\epsilon^2\), where typically \(\rho > \gamma\). The CIF produces an output \(x_{fused} = a\,x_{front} + b\,x_{back}\), whose signal-to-noise ratio (SNR) at the output is given by
% \begin{equation}
% \mathrm{SNR}_{\mathrm{out}} = \mathrm{SNR}_{\mathrm{in}} \cdot \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma},
% \label{eq:snr}
% \end{equation}
% where \(\mathrm{SNR}_{\mathrm{in}} = \sigma_s^2 / \sigma_\epsilon^2\).

% When \(ab < 0\), the term \(2ab\,\rho < 0\) in the numerator helps attenuate common-mode signal components, while \(2ab\,\gamma\) in the denominator reduces the effectiveness of noise cancellation, leading to \(\frac{a^2 + b^2}{(a + b)^2} > 1\), which indicates suppression of shared disturbances. On the other hand, when \(ab > 0\) and \(\rho > \gamma\), signal components are reinforced more than noise, ensuring \(\mathrm{SNR}_{\mathrm{out}} > \mathrm{SNR}_{\mathrm{in}}\). This demonstrates that CIF is effective both in suppressing noise and in enhancing signal content.

\textbf{Optimizing SNR via CIF:} Let two observed signals be \( x_1 = s_1 + \epsilon_1 \) and \( x_2 = s_2 + \epsilon_2 \), where \( s_1, s_2 \) are zero-mean useful signals with variance \( \sigma_s^2 \) and correlation coefficient \( \rho \), and \( \epsilon_1, \epsilon_2 \) are zero-mean noise components with variance \( \sigma_\epsilon^2 \) and correlation coefficient \( \gamma \). Assume that the signal and noise components are mutually uncorrelated. When applying the CIF operation via a linear combination \( y = a x_1 + b x_2 \), the output signal-to-noise ratio (SNR) becomes (details in Appendix~\ref{prove_CIF}):
\begin{equation}
\mathrm{SNR}_{\text{out}} = \mathrm{SNR}_{\text{in}} \cdot \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma}.
\label{eq:snr_gain}
\end{equation}

where \(\mathrm{SNR}_{\mathrm{in}} = \sigma_s^2 / \sigma_\epsilon^2\). When the numerator exceeds the denominator (i.e., 
\(\frac{a^2 + b^2 + 2ab\rho}{a^2 + b^2 + 2ab\gamma} > 1\)),
the SNR improves. This phenomenon occurs in two distinct modes: the \emph{Difference Mode} (\(ab < 0\) and \(\rho < \gamma\)) and the \emph{Cooperative Mode} (\(ab > 0\) and \(\rho > \gamma\)). In the Difference Mode, the correlation of noise sources (e.g., ocular artifacts) is higher than that of the signal, enhancing the SNR by suppressing correlated noise. In the Cooperative Mode, task-related brain regions exhibit synchronized activity while noise remains uncorrelated, leading to an increase in SNR by constructively accumulating and amplifying task-relevant signals. 
Both modes optimize the SNR by adjusting parameters $a$ and $b$, showcasing CIF's ability to suppress noise and enhance the signal under varying correlations.

% Both modes optimize the SNR adaptively by adjusting parameters \(a\) and \(b\), demonstrating CIF’s ability to suppress structured noise and enhance the target signal under varying correlation conditions.


% \begin{equation}
% \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma} > 1,
% \label{eq:snr_gain}
% \end{equation}

% In both the \emph{difference mode} and \emph{cooperative mode}, the inequality in equation \eqref{eq:snr_gain} holds, indicating that the output SNR improves relative to the input. The difference lies in the specific conditions for each mode:

% - In the \emph{difference mode}, when \( ab < 0 \) and \( \rho < \gamma \) — typically observed when noise sources (e.g., ocular artifacts) are more correlated than the signal — this results in effective suppression of the correlated noise, leading to an increase in SNR.

% - In the \emph{cooperative mode}, when \( ab > 0 \) and \( \rho > \gamma \) — a condition typically met when task-related brain regions show synchronized activity while noise remains relatively uncorrelated — the linear fusion amplifies the task-relevant signals, enhancing the SNR through constructive accumulation of the signal components.

% Thus, in both cases, CIF improves the signal-to-noise ratio under the appropriate conditions.



% \begin{equation}
% \mathrm{SNR}_{\text{out}} = \mathrm{SNR}_{\text{in}} \cdot \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma}.
% \label{eq:snr_gain}
% \end{equation}

% In the \emph{difference mode}, if \( ab < 0 \) and \( \rho < \gamma \) — which commonly occurs when noise sources (e.g., ocular artifacts) are more correlated than the underlying signal — then the following inequality holds:
% \begin{equation}
% \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma} > 1
% \label{eq:snr_inequality}
% \end{equation}
% which implies \( \mathrm{SNR}_{\text{out}} > \mathrm{SNR}_{\text{in}} \). This demonstrates that CIF can effectively suppress correlated noise and improve the signal-to-noise ratio under appropriate conditions.

% In the \emph{cooperative mode}, if \( ab > 0 \) and \( \rho > \gamma \) — a condition typically observed when task-related brain regions exhibit synchronized activity while noise sources remain relatively uncorrelated — then the following inequality holds:
% \begin{equation}
% \frac{a^2 + b^2 + 2ab\,\rho}{a^2 + b^2 + 2ab\,\gamma} > 1,
% \label{eq:snr_coop}
% \end{equation}
% indicating an improvement in output SNR relative to the input. In this case, the linear fusion constructively accumulates shared signal components across channels, amplifying task-relevant patterns, while the contributions of uncorrelated noise remain relatively incoherent and thus less amplified. This makes the cooperative mode particularly suitable for enhancing event-related potentials (ERPs) or distributed cortical oscillations that rely on spatial synchrony.



\textbf{Gradient Coupling Mechanism:} The coefficients $ a $ and $ b $ are optimized through gradient descent, where their updates are coupled due to shared dependencies on $ X_{i} $ and $ X_{j} $. The gradients as:
\begin{equation}
\frac{\partial \mathcal{L}}{\partial a} = \frac{\partial \mathcal{L}}{\partial X_{fused}} \cdot X_{i}, \quad \frac{\partial \mathcal{L}}{\partial b} = \frac{\partial \mathcal{L}}{\partial X_{fused}} \cdot X_{j}
\end{equation}

Specifically, the gradient computations of the loss function with respect to $a$ and $b$ include information from each other's signals, requiring their updates to simultaneously consider the influence of both forward and backward channels. This coupling mechanism enables the model to learn cross-channel interaction patterns, enhancing feature representation and generalization capability.
% CIF exhibits two adaptive modes based on the relationship between \( X_{\text{front}} \) and \( X_{\text{back}} \). In the \textbf{redundancy suppression mode}, when the two inputs share overlapping or noisy features, the gradients drive the coefficients \( a \) and \( b \) in opposite directions (\( a \uparrow, b \downarrow \)), effectively minimizing redundant contributions and suppressing noise. Conversely, in the \textbf{complementarity enhancement mode}, when \( X_{\text{front}} \) and \( X_{\text{back}} \) capture distinct yet synergistic information, the gradients encourage both \( a \) and \( b \) to increase simultaneously (\( a \uparrow, b \uparrow \)), amplifying the fused signal. This dynamic adjustment enables CIF to automatically tailor the fusion process to the data structure, optimizing representational efficiency without the need for manual tuning.

In Appendix~\ref{v_TCF}, we visualize scenarios with highly and generally correlated channel information.

% In Appendix~\ref{v_TCF}, we visualize scenarios with highly correlated channel information and those with generally correlated channel information. 
% These visualizations intuitively demonstrate the strong representation capability of our proposed method.

% In Figure \ref{fig_combined}, we visualize scenarios with highly correlated channel information and those with generally correlated channel information. These visualizations intuitively demonstrate the strong representation capability of our proposed method.


% % \begin{figure}[h]

% %     \centering
% %     \begin{subfigure}{0.48\textwidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{pic/EEG_Plot.pdf}
% %         \caption{}  % 自动显示 (a)
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}{0.48\textwidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{pic/EEG_Plot_change.pdf}
% %         \caption{}  % 自动显示 (b)
% %     \end{subfigure}
% %     \caption{Visual Comparison: When channel correlations are strong, (a) shows the visualization of the original time series, while (b) illustrates the results after applying the "imposed causal" operation.}
% %     \label{fig_strong}
% % \end{figure}

% % \begin{figure}[h]
% %     \centering

% %     \begin{subfigure}{0.48\textwidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{pic/APAVA_EEG_Plot.pdf}
% %         \caption{}  % 自动显示 (a)
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}{0.48\textwidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{pic/APAVA_EEG_Plot_change.pdf}
% %         \caption{}  % 自动显示 (b)
% %     \end{subfigure}
% %     \caption{Visual Comparison: When channel correlations are weak, (a) shows the visualization of the original time series, while (b) illustrates the results after applying the "imposed causal" operation.}
% %         \label{fig_weak}
% % \end{figure}


% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{pic/ADFTD-EEG_Plot_Original.pdf}
%         \caption{Original} 
%         \label{fig_strong_original}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{pic/ADFTD-EEG_Plot_change.pdf}
%         \caption{applying the Channel-Imposed Causality}
%         \label{fig_strong_imposed}
%     \end{subfigure}
    
%     \vspace{0.5cm} % 为了让上下两个图之间有一定间距
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{pic/APAVA_EEG_Plot_Original.pdf}
%         \caption{Original} 
%         \label{fig_weak_original}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{pic/APAVA_EEG_Plot_change.pdf}
%         \caption{ applying the Channel-Imposed Causality}
%         \label{fig_weak_imposed}
%     \end{subfigure}
    
%     \caption{Visual Comparison: (a) and (b) show the original and modified time series when channel correlations are strong, while (c) and (d) show the results for weak channel correlations. The modified time series are obtained by applying the Channel-Imposed Causality operation.}
%     \label{fig_combined}
% \end{figure}



% Our "Imposed Causality" theory is simple:
% Given an input tensor \( x_{\text{enc}} \) with shape \( (B, L, C) \), we extract the first \( n \) channels and the last \( n \) channels:
% \begin{equation}
% X_{\text{front}} = x_{\text{enc}}[:, :, :n]
% \end{equation}
% \begin{equation}
% X_{\text{back}} = x_{\text{enc}}[:, :, -n:]
% \end{equation}

% Then, we compute a weighted sum of these two parts:
% \begin{equation}
% X_{\text{added}} = a \cdot X_{\text{front}} + b \cdot X_{\text{back}}
% \end{equation}

% If \( t > 0 \), we replace the first \( n \) channels of \( x_{\text{enc}} \) with \( X_{\text{added}} \); otherwise, we replace the last \( n \) channels:

% % \begin{equation}
% % x_{\text{enc,new}}[:, :, :n] = X_{\text{added}}, \quad \text{if } t = 1
% % \end{equation}

% % \begin{equation}
% % x_{\text{enc,new}}[:, :, -n:] = X_{\text{added}}, \quad \text{if} t = -1
% % \end{equation}
% \begin{equation}
% x_{\text{enc,new}}[:, :, \pm n] = 
% \begin{cases} 
% X_{\text{added}} & \text{if } t = 1, \\
% X_{\text{added}} & \text{if } t = -1. 
% \end{cases}
% \end{equation}


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1\textwidth]{pic/main.pdf}
%     % \includegraphics[scale=1.5]{your_pdf_file.pdf}
%     \caption{arc }
%     \label{fig:your_label}
% \end{figure}


\subsection{HM-BiTCN Structure Design and Theoretical Analysis}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{pic/biTCN2.pdf}
    % \includegraphics[scale=1.5]{your_pdf_file.pdf}
    \caption{HM-BiTCN Architecture Diagram.}
    \label{fig:HM-BiTCN}
\end{figure}
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=1\textwidth]{pic/biTCN2.pdf}
%     % \includegraphics[scale=1.5]{your_pdf_file.pdf}
%     \caption{HM-BiTCN Architecture Diagram.}
%     \label{fig:your_label}
% \end{figure}


% ################原本的
% Modeling both short-term and long-term dependencies in time series data remains a significant challenge. While traditional convolutional neural networks (CNNs) are effective at extracting local features, their limited receptive fields make them less capable of capturing long-range dependencies. To overcome this limitation, the \textit{Hidden Mixed Bidirectional Temporal Convolutional Network (HM-BiTCN)} introduces a network architecture that integrates \textit{dilated convolution}, \textit{bidirectional convolution}, and \textit{residual connections}. This design enables the model to simultaneously capture both short-term and long-term temporal dependencies while preserving causality and enhancing feature extraction capabilities.


% \subsubsection{Dilated Convolution}

% Dilated convolution is a technique that expands the receptive field without significantly increasing computational cost. For a one-dimensional input sequence \( x = [x_1, x_2, \dots, x_T] \), the output of a dilated convolution can be expressed as:
% \begin{equation}
%     y(t) = \sum_{i=0}^{k-1} x(t + i \cdot d) \cdot w(i)
% \end{equation}
% where \( t \) represents the current time step, \( k \) is the kernel size, \( d \) is the dilation factor, and \( w(i) \) represents the weight at the \( i \)-th position in the convolutional kernel. By increasing the dilation factor \( d \), dilated convolution effectively expands the receptive field of each layer, allowing the network to capture dependencies over longer time spans. This approach enables the network to handle temporal dependencies across multiple scales without a significant increase in computational complexity.

% When stacking multiple dilated convolutional layers, the receptive field expands progressively. For the \( l \)-th layer, the receptive field \( r_l \) can be expressed as:
% \begin{equation}
%     r_l = k + (k - 1) \sum_{j=1}^{l-1} d_j
% \end{equation}
% where \( r_l \) is the receptive field of the \( l \)-th layer, and \( d_j \) represents the dilation factor at the \( j \)-th layer. By progressively increasing the dilation factor at each layer, the network captures temporal dependencies ranging from global to local scales, providing an effective mechanism for learning long-term dependencies in time series data.

% \subsubsection{Bidirectional Convolution}

% In addition to dilated convolutions, HM-BiTCN introduces a \textit{bidirectional convolution structure} to further enhance temporal dependency modeling. Traditional convolutional networks typically capture causal dependencies from past to present. However, in many real-world scenarios, future information is also essential for predicting the current state. To address this, the bidirectional convolution structure leverages both \textit{forward convolution} and \textit{backward convolution}, allowing the model to integrate past and future information, which improves its feature representation capabilities.

% \textit{Forward convolution} refers to the standard causal convolution that captures dependencies from past to present. Given an input sequence \( x(t) \), the forward convolution output is:
% \begin{equation}
%     y_{\text{forward}}(t) = \sum_{i=0}^{k-1} x(t - i \cdot d) \cdot w_{\text{forward}}(i)
% \end{equation}

% \textit{Backward convolution}, on the other hand, operates on the reversed input sequence to capture dependencies from the future to the present. Let the flipped input sequence be defined as \( x_{\text{flip}}(t) = x(T - t) \), then the backward convolution output is:
% \begin{equation}
%     y_{\text{backward}}(t) = \sum_{i=0}^{k-1} x_{\text{flip}}(t - i \cdot d) \cdot w_{\text{backward}}(i) = \sum_{i=0}^{k-1} x(T - (t - i \cdot d)) \cdot w_{\text{backward}}(i)
% \end{equation}
% % This can also be expressed as:
% % \begin{equation}
% %     y_{\text{backward}}(t) = \sum_{i=0}^{k-1} x(T - (t - i \cdot d)) \cdot w_{\text{backward}}(i)
% % \end{equation}

% In HM-BiTCN, the forward and backward convolutions are handled by separate convolutional layers, convforward and convbackward, respectively. The outputs of these two convolutions are then combined to produce the final bidirectional convolution output. 
% \begin{equation}
%     y_{\text{bi}}(t) = y_{\text{forward}}(t) + y_{\text{backward}}(t)
% \end{equation}
% By incorporating bidirectional convolutions, HM-BiTCN effectively utilizes both past and future information, which significantly enhances the model’s ability to capture complex temporal dependencies.

% \subsubsection{Multi-Scale Feature Learning and Residual Connections}

% To further improve the model's capacity to capture dependencies at different temporal scales, HM-BiTCN incorporates \textit{multi-scale feature learning} and \textit{residual connections}.

% \textbf{Multi-scale feature learning}: Different dilation factors are applied at different layers to capture temporal dependencies at varying scales. Lower layers use larger dilation factors to capture long-range dependencies, while higher layers use smaller dilation factors to focus on short-range dependencies. This hierarchical approach allows the network to process temporal dependencies from a global to a local perspective, extracting broader patterns at the initial layers and refining finer details at the later layers. As a result, the network is more adaptable to a wide range of time series tasks.

% \textbf{Residual connections}: Residual connections are introduced between the dilated convolutional layers to facilitate the efficient flow of information through the network. The residual connection is defined as:
% \begin{equation}
%     y = F(x) + x
% \end{equation}
% where \( F(x) \) is the convolutional output, and \( x \) is the input. This design alleviates the vanishing gradient problem and improves the overall stability of the network during training.


%  HM-BiTCN combines dilated convolution, bidirectional convolution, multi-scale feature learning, and residual connections, enabling the network to efficiently capture dependencies across multiple temporal scales while preserving causality. This architecture allows the model to effectively learn both long-term and short-term dependencies in time series data, making it particularly well-suited for tasks that require complex temporal modeling.


% 我们的

% Modeling both short-term and long-term dependencies in time series data remains a significant challenge. While traditional CNNs are effective at extracting local features, their limited receptive fields make them less capable of capturing long-range dependencies. To overcome this limitation, the \textit{Hidden Mixed Bidirectional Temporal Convolutional Network (HM-BiTCN)} introduces a network architecture that integrates \textit{dilated convolution}, \textit{bidirectional convolution}, and \textit{residual connections}. This design enables the model to simultaneously capture both short-term and long-term temporal dependencies while preserving causality and enhancing feature extraction capabilities. \textbf{Our goal is to simplify the structure as much as possible while improving its interpretability.}

% Compared to the Transformer-based models, the TCN~\cite{bai2018empirical,wang2024contrast} circumvents the aforementioned issues through explicit structural design: its causal convolutions ensure that temporal dependencies strictly follow the forward propagation direction, thereby preventing future information leakage; dilated convolutions \textbf{explicitly} control the receptive field range via exponentially increasing dilation factors, enabling controllable modeling of long-range dependencies.  This explicit modeling mechanism not only endows the model with a clear temporal logic , but also allows the integration of domain-specific priors through structural constraints .
% Modeling both short-term and long-term dependencies in time-series data remains a significant challenge. While traditional CNNs are effective at extracting local features, their limited receptive fields make it difficult to capture long-range dependencies. Transformer-based methods, while excelling at capturing long-term dependencies, often suffer from poor interpretability and unclear causal relationships due to their implicit modeling characteristics and relatively complex structures, which is especially problematic in medical time-series classification. 
% Modeling both short-term and long-term dependencies in time-series data remains a challenge. Traditional CNNs are effective at extracting local features, but their limited receptive fields make it difficult to capture long-range dependencies. Transformer-based methods excel at capturing long-term dependencies, but their implicit modeling and complex structures often lead to poor interpretability and unclear causal relationships, which is particularly problematic in medical time-series classification.
% Modeling short-term and long-term dependencies in time series data remains challenging. While traditional CNNs capture local features well, their limited receptive fields hinder long-range dependency learning. Transformer-based methods model long-term dependencies effectively but lack interpretability due to their implicit and complex design — a key issue in medical time-series classification.
% To address these limitations, temporal convolutional networks (TCNs) use causal convolutions for explicit temporal modeling and dilated convolutions to expand the receptive field, overcoming the constraints of traditional CNNs.
Modeling short-term and long-term dependencies in time series data is challenging. Traditional CNNs excel at capturing local features but have limited receptive fields, hindering long-range dependency learning. Transformer-based methods effectively model long-term dependencies, but their complex design lacks interpretability, which is a key issue in medical time-series classification.To address these limitations, TCNs use causal convolutions for explicit temporal modeling and dilated convolutions to expand the receptive field, overcoming the constraints of traditional CNNs.
% To address these issues, TCN explicitly captures temporal dependencies using causal convolutions and expands the receptive field through dilated convolutions, effectively overcoming the receptive field limitations of traditional CNNs. 
Building on the advantages of TCN, we propose the HM-BiTCN, which combines the benefits of dilated convolutions, bidirectional causal convolution, and residual connections. This approach allows for better capture of temporal dependencies while preserving causality. \textbf{Our goal is to simplify the model structure through explicit design principles while improving its interpretability. }
% Compared to Transformer-based methods, HM-BiTCN demonstrates significant advantages in model transparency, structural simplicity, and the balance between short- and long-term dependency modeling.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{pic/biTCN2.pdf}
%     % \includegraphics[scale=1.5]{your_pdf_file.pdf}
%     \caption{HM-BiTCN Architecture Diagram.}
%     \label{fig:your_label}
% \end{figure}


% \subsubsection{Dilated Convolution}

% Dilated convolution is a technique that expands the receptive field without significantly increasing computational cost~\cite{yu2015multi}. For a one-dimensional input sequence \( x = [x_1, x_2, \dots, x_T] \), the output of a dilated convolution can be expressed as \( y(t) = \sum_{i=0}^{k-1} x(t + i \cdot d) \cdot w(i) \), where \( t \) represents the current time step, \( k \) is the kernel size, \( d \) is the dilation factor, and \( w(i) \) represents the weight at the \( i \)-th position in the convolutional kernel. By increasing the dilation factor \( d \), dilated convolution effectively expands the receptive field of each layer, allowing the network to capture dependencies over longer time spans. This approach enables the network to handle temporal dependencies across multiple scales without a significant increase in computational complexity. When stacking multiple dilated convolutional layers, the receptive field expands progressively. For the \( l \)-th layer, the receptive field \( r_l \) can be expressed as \( r_l = k + (k - 1) \sum_{j=1}^{l-1} d_j \), where \( r_l \) is the receptive field of the \( l \)-th layer, and \( d_j \) represents the dilation factor at the \( j \)-th layer. By progressively increasing the dilation factor at each layer, the network captures temporal dependencies ranging from global to local scales, providing an effective mechanism for learning long-term dependencies in time series data.
\subsubsection{Dilated Convolution}

Dilated convolution expands the receptive field without significantly increasing computational cost~\cite{yu2015multi}. For a 1D input sequence $ x = [x_1, x_2, \dots, x_T] $, its output is defined as $ y(t) = \sum_{i=0}^{k-1} x(t + i \cdot d) \cdot w(i) $, where $ t $ is the current time step, $ k $ is the kernel size, $ d $ is the dilation factor, and $ w(i) $ is the weight at the $ i $-th position in the kernel. Increasing $ d $ effectively enlarges the receptive field, enabling the network to capture longer-term temporal dependencies. 
When stacking multiple dilated convolutional layers, the receptive field grows progressively. For the $ l $-th layer, the receptive field $ r_l $ can be expressed as $ r_l = k + (k - 1) \sum_{j=1}^{l-1} d_j $, where $ d_j $ is the dilation factor of the $ j $-th layer. By gradually increasing $ d_j $, the network captures temporal dependencies across both global and local scales, offering an effective way to model long-term dependencies in time series.

% \subsubsection{Bidirectional Convolution}

% % In addition to dilated convolutions, in spired by the previous work~\cite{hanson2018bidirectional,hu2024specslice,yin2025degradation}, HM-BiTCN introduces a \textit{bidirectional convolution structure} to further enhance temporal dependency modeling. 
% In addition to dilated convolutions, inspired by previous works that utilize bidirectional temporal structures~\cite{hanson2018bidirectional, hu2024specslice, yin2025degradation}, HM-BiTCN introduces a \textit{bidirectional convolution structure} to further enhance temporal dependency modeling.
% The bidirectional convolution structure leverages both \textit{forward convolution} and \textit{backward convolution}, allowing the model to integrate past and future information, which improves its feature representation capabilities. \textit{Forward convolution} refers to the standard causal convolution that captures dependencies from past to present. Given an input sequence \( x(t) \), the forward convolution output is \( y_{\text{forward}}(t) = \sum_{i=0}^{k-1} x(t - i \cdot d) \cdot w_{\text{forward}}(i) \). \textit{Backward convolution}, on the other hand, operates on the reversed input sequence to capture dependencies from the future to the present. Let the flipped input sequence be defined as \( x_{\text{flip}}(t) = x(T - t) \), then the backward convolution output is \( y_{\text{backward}}(t) = \sum_{i=0}^{k-1} x_{\text{flip}}(t - i \cdot d) \cdot w_{\text{backward}}(i) = \sum_{i=0}^{k-1} x(T - (t - i \cdot d)) \cdot w_{\text{backward}}(i) \). In HM-BiTCN, the forward and backward convolutions are handled by separate convolutional layers, convforward and convbackward, respectively. The outputs of these two convolutions are then combined to produce the final bidirectional convolution output: \( y_{\text{bi}}(t) = y_{\text{forward}}(t) + y_{\text{backward}}(t) \). By incorporating bidirectional convolutions, HM-BiTCN effectively utilizes both past and future information, which significantly enhances the model’s ability to capture complex temporal dependencies.
% \subsubsection{Bidirectional Causal Convolution Structure}

% In addition to dilated convolutions, inspired by prior work utilizing bidirectional temporal structures~\cite{hanson2018bidirectional, hu2024specslice, yin2025degradation}, HM-BiTCN introduces a \textit{bidirectional causal convolution structure} to more comprehensively model temporal dependencies. Unlike traditional TCNs that employ only unidirectional causal convolutions (forward-in-time modeling), our architecture applies causal convolutions in both forward and backward directions while preserving causality. This design enables the model to fully exploit temporal dependencies from both past and future directions without leaking future information.
% Specifically, the \textit{forward causal convolution} processes the input sequence in chronological order, ensuring that each output depends only on the current and preceding time steps. Given an input sequence $x(t)$, the output is computed as $y_{\text{forward}}(t) = \sum_{i=0}^{k-1} x(t - i \cdot d) \cdot w_{\text{forward}}(i)$.
% At the same time, we apply a \textit{backward causal convolution} to the reversed input sequence. This operation also respects causality by relying only on the current and "past" time steps in the flipped sequence — which correspond to future moments in the original sequence. Let the flipped input be defined as $x_{\text{flip}}(t) = x(T - t)$. The output of the backward convolution is then given by $y_{\text{backward}}(t) = \sum_{i=0}^{k-1} x_{\text{flip}}(t - i \cdot d) \cdot w_{\text{backward}}(i) = \sum_{i=0}^{k-1} x(T - (t - i \cdot d)) \cdot w_{\text{backward}}(i)$.
% In HM-BiTCN, these two causal convolutions are implemented using separate convolutional layers (convforward and convbackward), and their outputs are summed to produce the final bidirectional convolution result: $y_{\text{bi}}(t) = y_{\text{forward}}(t) + y_{\text{backward}}(t)$.
% Through this design, HM-BiTCN strictly maintains causality while effectively integrating contextual information from both past and future directions. Compared to conventional unidirectional causal modeling approaches, this bidirectional structure offers enhanced modeling capacity and improved predictive performance.
\subsubsection{Bidirectional Causal Convolution Structure}

In addition to dilated convolutions, HM-BiTCN introduces a \textit{bidirectional causal convolution structure}, inspired by prior bidirectional temporal modeling approaches~\cite{hanson2018bidirectional, hu2024specslice, yin2025degradation}. Unlike traditional TCNs that use only forward causal convolutions, our architecture applies causal convolutions in both forward and backward directions, enabling the model to capture dependencies from both past and future contexts while strictly preserving causality.
The \textit{forward causal convolution} processes the input sequence $x(t)$ in chronological order, producing output $y_{\text{forward}}(t) = \sum_{i=0}^{k-1} x(t - i \cdot d) \cdot w_{\text{forward}}(i)$, which depends only on current and past inputs. 
For the \textit{backward causal convolution}, we first reverse the input sequence as $x_{\text{flip}}(t) = x(T - t)$, and then apply a causal convolution over this flipped sequence. This ensures that the model captures future-directed dependencies without introducing information leakage. The output is given by $y_{\text{backward}}(t) = \sum_{i=0}^{k-1} x(T - (t - i \cdot d)) \cdot w_{\text{backward}}(i)$.
These two operations are implemented using separate convolutional layers (convforward and convbackward), and their outputs are summed to form the final bidirectional result: $y_{\text{bi}}(t) = y_{\text{forward}}(t) + y_{\text{backward}}(t)$.
By integrating both directions under strict causality constraints, HM-BiTCN achieves superior temporal dependency modeling compared to unidirectional causal approaches.

\subsubsection{Multi-Scale Feature Learning and Residual Connections}
To further improve the model's capacity to capture dependencies at different temporal scales, HM-BiTCN incorporates \textit{multi-scale feature learning} and \textit{residual connections}. 
Multi-scale Feature Learning:
In HM-BiTCN, we employ a hierarchy of dilation factors that decrease layer by layer to capture temporal dependencies at multiple scales. Lower layers use larger dilation factors to expand the receptive field, aggregating long‐range information and smoothing short‐term noise in highly redundant medical time series; higher layers use smaller dilation factors to focus on local dependencies and capture fine‐grained features. This coarse‐to‐fine, global‐to‐local design enables the network to extract broad patterns in its initial layers and refine precise details in its later layers, thereby enhancing adaptability across a wide range of time series tasks. Residual connections:
Residual connections~\cite{he2016deep} are introduced between the dilated convolutional layers to facilitate the efficient flow of information through the network. The residual connection is defined as \( y = F(x) + x \), where \( F(x) \) is the convolutional output, and \( x \) is the input. This design alleviates the vanishing gradient problem and improves the overall stability of the network during training.

% \textbf{Multi-scale feature learning}: Different dilation factors are applied at different layers to capture temporal dependencies at varying scales. Lower layers use larger dilation factors to capture long-range dependencies, while higher layers use smaller dilation factors to focus on short-range dependencies. This hierarchical approach allows the network to process temporal dependencies from a global to a local perspective, extracting broader patterns at the initial layers and refining finer details at the later layers. As a result, the network is more adaptable to a wide range of time series tasks. \textbf{Residual connections}: Residual connections~\cite{he2016deep} are introduced between the dilated convolutional layers to facilitate the efficient flow of information through the network. The residual connection is defined as \( y = F(x) + x \), where \( F(x) \) is the convolutional output, and \( x \) is the input. This design alleviates the vanishing gradient problem and improves the overall stability of the network during training.

% In the design of HM-BiTCN, we employ dilation factors that decrease layer by layer—first using larger dilated convolutions to expand the receptive field, thereby aggregating long-range information and smoothing short-term noise in highly redundant medical time series; then using smaller dilated convolutions to capture fine-grained features.



==> sections/preliminaries.tex <==

We define the MedTS classification task as a supervised learning problem over time series data with hierarchical subject-level structure. The dataset is represented as \( \mathcal{D} = \{(x_i, y_i, s_i)\}_{i=1}^N \), where \( x_i \in \mathbb{R}^{T \times C} \) is the \(i\)-th sample with \(T\) time steps and \(C\) channels, \( y_i \in \{0,1\}^K \) is a multi-label vector over \(K\) categories, and \( s_i \in \mathbb{N} \) is the subject ID. Samples from the same subject share the same label, i.e., \( y_i = y_j, \forall x_i, x_j \in \mathcal{D}_s \), where \( \mathcal{D}_s \) represents the set of samples from subject \(s\). We consider two dataset partitioning strategies: (i) \textbf{Subject-Dependent Split}, where the dataset is split at the sample level such that samples from the same subject may appear in both training and test sets, which can cause information leakage and yield overly optimistic performance estimates; and (ii) \textbf{Subject-Independent Split}, where the dataset is split at the subject level, ensuring that each subject appears only in one of the train, validation, or test sets, simulating real-world diagnostic scenarios but introducing challenges due to inter-subject variability.
The goal is to train an encoder \( f_\theta: \mathbb{R}^{T \times C} \rightarrow \mathbb{R}^d \) to obtain a latent representation \( h_i = f_\theta(x_i) \), which is then passed to a classifier \( g_\phi \) to predict the label \( \hat{y}_i = g_\phi(h_i) \).
% The training objective is to minimize the loss function \( \mathcal{L} = \frac{1}{N} \sum_{i=1}^N \ell(\hat{y}_i, y_i) \), where \( \ell(\hat{y}_i, y_i) \) is the loss between the predicted and true labels.


==> sections/related.tex <==
% \textbf{Medical Time Series.}
% Medical time series analysis diverges fundamentally from general time series forecasting \cite{wu2022timesnet,lu2024cats} by prioritizing pathological signature decoding over temporal extrapolation, with modalities like EEG \cite{tangself,yangmanydg,quensemble}, ECG \cite{xiao2023deep,wang2023hierarchical,kiyasseh2021clocs}, and EMG [\cite{xiong2021deep,dai2022mseva}] encoding distinct clinical semantics.
% Existing deep learning analysis methods for medical time series cover a variety of models, including Convolutional Neural Networks (CNN)~\cite{lawhern2018eegnet}, Temporal Convolutional Networks (TCN)~\cite{bai2018empirical,wang2024contrast},  Long Short-Term Memory networks (LSTM)~\cite{nagabushanam2020retracted}, the Mamba algorithm~\cite{gu2023mamba,wang2024medformer}, and the Transformer architecture~\cite{wang2024medformer,zhu2025mtnet}. Each of these methods has unique advantages and is suitable for parsing different modalities of medical time series data, such as EEG, ECG, and EMG, to uncover the complex clinical semantics embedded within them.
\textbf{Medical Time Series Classification.}
Medical time series analysis diverges fundamentally from general time series forecasting \cite{wu2022timesnet,lu2024cats} by prioritizing pathological signature decoding over temporal extrapolation, with modalities like EEG \cite{tangself,yangmanydg,quensemble}, ECG \cite{xiao2023deep,wang2023hierarchical,kiyasseh2021clocs}, and EMG [\cite{xiong2021deep,dai2022mseva}] encoding distinct clinical semantics. Early methods were dominated by compact CNNs such as EEGNet~\cite{lawhern2018eegnet}, which employs depthwise separable convolutions to efficiently extract spatio–temporal features while providing preliminary interpretability via feature‐map visualization. Subsequently, temporal convolutional networks (TCNs)~\cite{bai2018empirical,lin2019medical} leveraging dilated causal convolutions achieved parallelizable computation and extended receptive fields, surpassing LSTM‐based approaches~\cite{zhou2016attention,shen2016neural,hochreiter1997long} on multiple medical signal classification benchmarks.  Hybrid architectures such as EEG‐Conformer~\cite{song2022eeg} combined convolutional front‐ends with Transformer self‐attention to capture both local and global dependencies and enabled attention‐based interpretability.  More recently, fine-grained Transformer models such as Medformer~\cite{wang2024medformer} introduced cross-channel tokenization and dual-stage self-attention, setting new SOTA accuracy on several public datasets.  The latest MedGNN ~\cite{fan2025medgnn} further augments attention mechanisms with multi‐resolution graph learning to jointly model spatial multi‐scale channel dependencies and temporal dynamics.  Although Transformer models have significantly improved classification accuracy, their complexity, especially due to deep architectures and multi-layer attention mechanisms, results in reduced interpretability. In clinical applications, where model transparency and reliability are essential, it is imperative to strike a balance between high accuracy and explainability.



% \textbf{Transformers for Time Series.}
% Transformer architectures have exhibited remarkable learning proficiency across diverse domains including temporal data analysis, where they have been extensively adapted for forecasting and classification tasks. Current research on Transformer-based temporal modeling predominantly focuses on two technical directions: (1) enhancing token embedding techniques to better capture temporal dynamics, and (2) refining attention mechanisms to model temporal dependencies effectively, often through hybrid approaches. Representative works include PatchTST~\cite{nie2022time}, which employs single-variable temporal patch segmentation for sequence representation; Autoformer~\cite{wu2021autoformer} and Informer~\cite{zhou2021informer}, which develop enhanced attention mechanisms with sub-quadratic complexity; and hybrid architectures like Crossformer~\cite{zhang2022crossformer} and iTransformer~\cite{liu2023itransformer} that integrate both strategies.
% For temporal feature extraction, methods such as Pyraformer~\cite{liu2021pyraformer} and Scaleformer~\cite{shabani2022scaleformer} leverage multi-scale embedding strategies to simultaneously model granular and holistic temporal patterns. Recent innovations like Medformer~\cite{wang2024medformer} propose cross-variate patch embeddings to capture inter-channel dependencies, while MedGNN~\cite{fan2025medgnn} integrates graph neural networks with multi-resolution temporal analysis for dynamic feature learning.

\textbf{Implicit modeling strategies in Transformer-based temporal methods.}
In time series analysis, Transformer-based models implicitly learn complex dependencies through diversified architectural designs: the vanilla Transformer~\cite{vaswani2017attention} first introduced multi-head self-attention and sinusoidal positional encoding to model temporal correlations globally; Informer~\cite{zhou2021informer} employs ProbSparse attention to select key time steps and compress sequence length, thereby reducing the computational cost of long-range dependencies; Reformer~\cite{kitaev2019reformer} incorporates Locality-Sensitive Hashing (LSH) to reduce attention complexity to \(\mathcal{O}(L\log L)\), making it suitable for ultra-long sequences; Autoformer~\cite{wu2021autoformer} proposes an Auto-Correlation mechanism that aggregates periodic subsequences to enhance the implicit capture of cyclic patterns; FEDformer~\cite{zhou2022fedformer} performs seasonal–trend decomposition in the frequency domain and uses compressed Fourier coefficients to enable cross-frequency attention interactions; Crossformer~\cite{zhang2022crossformer} designs a two-stage attention mechanism across time and feature dimensions to implicitly fuse multivariate spatiotemporal couplings; iTransformer~\cite{liu2023itransformer} innovatively treats time steps as channel dimensions and applies standard attention to implicitly learn nonlinear inter-variable relationships; PatchTST~\cite{nie2022time} segments continuous time steps into patch-based tokens and uses a combination of local and global attention to capture multi-scale temporal patterns; Medformer~\cite{wang2024medformer} introduces multi-granularity patch embeddings and cross-channel attention for medical signals, implicitly modeling the heterogeneous couplings of physiological metrics; and MedGNN~\cite{fan2025medgnn} combines graph attention with frequency-differential networks to incorporate medical topological priors into implicit spatiotemporal dependency learning. Although these variants enhance time series modeling via attention-based techniques, their reliance on high-dimensional weight matrices to implicitly encode dependencies between time steps and variables hinders interpretability. This limitation is particularly severe in medical applications, where it undermines the trustworthiness of high-risk tasks such as disease diagnosis and risk prediction.

% \textbf{Implicit modeling in Transformer-based methods.}
% Transformer-based time series models such as vanilla Transformer~\cite{vaswani2017attention}, Informer~\cite{zhou2021informer}, Reformer~\cite{kitaev2019reformer}, Autoformer~\cite{wu2021autoformer}, FEDformer~\cite{zhou2022fedformer}, Crossformer~\cite{zhang2022crossformer}, iTransformer~\cite{liu2023itransformer}, PatchTST~\cite{nie2022time}, Medformer~\cite{wang2024medformer} and MedGNN~\cite{fan2025medgnn} rely on self-attention and positional encoding to \textbf{implicitly} learn temporal and cross-variable dependencies. Each variant tweaks attention (e.g., sparse queries, LSH, frequency decomposition, multi-scale patches and graph priors) to boost efficiency and capture richer patterns, yet they still hide their dependency logic within high-dimensional weight matrices, which limits interpretability, especially in critical medical applications.
% Compared to the Transformer-based models, the TCN~\cite{bai2018empirical,wang2024contrast} circumvents the aforementioned issues through explicit structural design: its causal convolutions ensure that temporal dependencies strictly follow the forward propagation direction, thereby preventing future information leakage; dilated convolutions \textbf{explicitly} control the receptive field range via exponentially increasing dilation factors, enabling controllable modeling of long-range dependencies.  This explicit modeling mechanism not only endows the model with a clear temporal logic , but also allows the integration of domain-specific priors through structural constraints . 
% % This study combines TCN with the Causal Influence Framework (CIF) based on their dual advantages: (1) the explicit dependency paths provide medical interpretability, meeting the transparency requirements of clinical decision-making; (2) the controllable expansion of the receptive field enables simultaneous capture of both short- and long-term patterns, avoiding the attention mechanism's oversensitivity to local noise. This design achieves a balance between performance and trustworthiness in medical time-series analysis, offering more reliable solutions for high-risk scenarios.


==> sections/result.tex <==
\subsection{Results of Subject-Dependent}
\label{sub:subject_dependent_result}
% In the Subject-Dependent setup, the training, validation, and test sets are divided based on samples. All samples from all subjects are first randomly shuffled and then distributed into the respective sets according to a predetermined ratio, allowing samples from the same subject to appear in all three sets simultaneously. While this method is helpful for quickly assessing whether the dataset exhibits cross-subject features and demonstrates the upper limit of learnability, its application in real-world MedTS-based disease diagnosis scenarios is \textbf{relatively limited}.
% In the \textit{Subject-Dependent} setup, all samples are randomly shuffled and split into training, validation, and test sets according to a fixed ratio, allowing samples from the same subject to appear in multiple sets. This approach helps evaluate the upper bound of learnability and cross-subject feature presence, but has limited applicability in real-world MedTS-based disease diagnosis scenarios.
\input{table/subject_dependent}
To further validate our proposed method, we reproduced 12 baseline approaches. Table~\ref{tab:subject-dependent-report} presents a comparison of the \textbf{reported} experimental results for these methods, while Table~\ref{tab:subject-dependent_reproduce} in Appendix~\ref{app:reproduce_result} provides detailed results from our \textbf{reproduction} of the 12 methods. The experimental results demonstrate that by incorporating our proposed CIF method into the Medformer model, we not only achieve significantly better performance than the original methods, but also outperform the current state-of-the-art (SOTA) approach, MedGNN. These findings strongly confirm the effectiveness and superiority of our method.

\subsection{Results of Subject-Independent}
\label{sub:subject_independent_result}


In the Subject-Independent setup, the training, validation, and test sets are split based on subjects. All subjects and their corresponding samples are distributed into these three sets according to a predetermined ratio or subject IDs. Samples from the same subject exclusively appear in one of the three sets. This setup simulates real-world MedTS-based disease diagnosis, aiming to train a model on subjects with known labels and then test it on unseen subjects to determine if they have a specific disease. All five datasets are evaluated under this setup.

Table~\ref{tab:subject-independent-report} presents the results \textbf{reported} by various methods in the subject-independent setting, while Table~\ref{tab:subject-independent-reproduce} shows the results of our \textbf{reproduction} of these methods. Our method achieves the highest scores in six metrics across four out of the five datasets. For the PTB-XL dataset, compared to the results reported by other methods, our approach achieves the highest AUROC and AUPRC score and ranks second in Accuracy. When compared to the results of our reproduction, our method ranks first in Accuracy, Precision, AUROC, and AUPRC, and second in Recall.
Additionally, it is worth noting that in the subject-independent setup, the F1 score of ADFTD is 55.42\%, which is significantly lower than the 99.59\% achieved in the subject-dependent setup. This comparison highlights the challenges of the subject-independent setup, \textbf{which better simulates real-world scenarios}.

 \input{table/ind_res_original}

\subsubsection{Efficiency Analysis}
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
       \includegraphics[width=\linewidth]{pic/qipao_APAVA.pdf}
        \caption{APAVA-Subject}  % 自动显示 (a)
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \centering
          \includegraphics[width=\linewidth]{pic/qipao_TDBrain.pdf}
        \caption{TDBRAIN-Subject}  % 自动显示 (b)
    \end{subfigure}
    \caption{Model effectiveness and efficiency comparison on
two datasets under the Subject-based setup.} 
        \label{fig_APAVA_TDBrain}
\end{figure}
We evaluate the model efficiency in terms of accuracy, training speed, and memory footprint using two datasets: APAVA and TDBRAIN. In Figure~\ref{fig_APAVA_TDBrain}, a marker closer to the upper-left corner indicates higher accuracy and faster training speed, while a smaller marker area corresponds to lower memory usage. The results show that HM-BiTCN achieves the best overall performance among all baseline methods, demonstrating its high efficiency and reliability across different application scenarios.

\subsection{Ablation Study}
\label{sub:Ablation}
\input{sections/Ablation}




==> table/Ablation/Ablation_ADFTD.tex <==

% \begin{table}[htp]
% \arraystretch{1.0}

% \centering
% \caption{Ablation study of CIF structure hyperparameters on ADFTD dataset (19 Channels).We use \includegraphics[width=1em]{pic/learnable.pdf} to represent learnable parameters, and \includegraphics[width=1em]{pic/frozen.pdf} to represent non-learnable parameters.}
% \begin{tabular}{cccc*{6}{>{\centering\arraybackslash}p{1.1cm}}}
% \toprule
%  \multicolumn{1}{c}{\textbf{t \uparrow}} & \multicolumn{1}{c}{\textbf{n \uparrow}} & \multicolumn{1}{c}{\textbf{a \uparrow}}  & \multicolumn{1}{c}{\textbf{b \uparrow}}  &\multicolumn{1}{c}{\textbf{Accuracy \uparrow}} & \multicolumn{1}{c}{\textbf{Precision \uparrow}} & \multicolumn{1}{c}{\textbf{Recall \uparrow}} & \multicolumn{1}{c}{\textbf{F1 score \uparrow}} & \multicolumn{1}{c}{\textbf{AUROC \uparrow}} & \multicolumn{1}{c}{\textbf{AUPRC \uparrow}}  \\
% \midrule

% - & - 
% & -
% & -
% & 52.05\std{2.22} & 50.45\std{3.00} & 50.40\std{2.55} & 49.48\std{2.70} & 69.43\std{2.84} & 50.99\std{3.15} \\


% 1 & 10 
% & -0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.30 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 57.33\std{0.95}& 54.06\std{1.47}& 54.44\std{1.33}& 53.73\std{1.47}& 74.82\std{1.36}& 58.24\std{1.78} \\

% 1 & 10 
% & -0.25 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.40 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 57.08\std{1.46}& 53.31\std{0.98}& 53.24\std{1.14}& 52.87\std{0.98}& 73.77\std{1.28}& 56.86\std{1.47} \\

% 1 & 11 
% & -0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.30 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 56.68\std{1.30}& 53.04\std{2.00}& 53.45\std{2.03}& 52.84\std{2.30}& 73.81\std{1.55}& 57.34\std{1.46} \\

% % 1 & 11 
% % & -0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% % & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% % & 56.01\std{0.73}& 53.10\std{0.64}& 53.49\std{0.76}& 53.10\std{0.61}& 73.29\std{0.42}& 56.61\std{0.19} \\

% % 1 & 11 
% % & -0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% % & -0.30 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% % & 56.89\std{0.93}& 53.84\std{0.45}& 54.16\std{0.49}& 53.56\std{0.75}& 74.26\std{0.54}& 57.57\std{0.97} \\




% 1 & 10 
% & -0.19 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & -0.27 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & \textbf{58.56\std{0.93}}& \textbf{55.65\std{0.81}}& \textbf{55.86\std{0.79}}& \textbf{55.42\std{0.82}}& \textbf{76.07\std{0.59}}& \textbf{59.75\std{0.67}} \\

% 1 & 7 
% & \;0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & -0.60 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 56.36\std{0.58}& 53.91\std{1.10}& 54.34\std{1.03}& 53.78\std{0.91}& 74.19\std{0.69}& 56.62\std{1.28} \\

% 1 & 9 
% & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & -0.60 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 55.20\std{1.50}& 53.05\std{1.14}& 53.21\std{1.06}& 52.76\std{1.02}& 73.09\std{1.13}& 55.50\std{1.71} \\

% 1 & 10 
% & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 57.11\std{0.92}& 55.04\std{1.43}& 55.53\std{1.57}& 54.58\std{1.29}& 75.13\std{1.33}& 58.47\std{1.43} \\

% % 1 & 10 
% % & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% % & -0.30 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% % & 56.84\std{1.49}& 53.77\std{0.78}& 54.10\std{0.81}& 53.71\std{0.91}& 74.26\std{1.31}& 57.26\std{1.60} \\

% % 1 & 10 
% % & -0.18 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% % & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% % & 57.20\std{1.19}& 54.02\std{0.97}& 54.05\std{0.56}& 53.43\std{0.56}& 74.53\std{0.54}& 57.57\std{0.52} \\

% % 1 & 10 
% % & -0.18 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% % & -0.30 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% % & 58.44\std{1.03}& 54.41\std{1.84}& 54.84\std{1.62}& 54.12\std{2.05}& 75.17\std{1.18}& 58.33\std{1.53} \\

% 1 & 11 
% & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & -0.30 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 57.83\std{1.16}& 54.32\std{1.22}& 54.51\std{1.18}& 54.01\std{1.21}& 74.74\std{1.12}& 57.96\std{1.08} \\

% 1 & 11 
% & -0.18 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & -0.25 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 57.00\std{1.32}& 53.00\std{2.28}& 53.17\std{1.94}& 52.32\std{2.19}& 73.97\std{1.89}& 57.00\std{1.93} \\




% \bottomrule
% \end{tabular}
% \label{tab:ablation}
% \end{table}



\begin{table}[htp]
% \arraystretch{1.0}
\centering
\caption{Ablation study of CIF structure hyperparameters on ADFTD dataset (19 Channels). We use \includegraphics[width=1em]{pic/learnable.pdf} to represent learnable parameters, and \includegraphics[width=1em]{pic/frozen.pdf} to represent non-learnable parameters.}

\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc*{6}{>{\centering\arraybackslash}p{1.1cm}}}
\toprule
\multicolumn{1}{c}{\textbf{t }} & \multicolumn{1}{c}{\textbf{n }} & \multicolumn{1}{c}{\textbf{a }}  & \multicolumn{1}{c}{\textbf{b }}  &\multicolumn{1}{c}{\textbf{Accuracy $\uparrow$}} & \multicolumn{1}{c}{\textbf{Precision $\uparrow$}} & \multicolumn{1}{c}{\textbf{Recall $\uparrow$}} & \multicolumn{1}{c}{\textbf{F1 score $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUROC $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUPRC $\uparrow$}}  \\
\midrule

- & - & - & - & 52.05\std{2.22} & 50.45\std{3.00} & 50.40\std{2.55} & 49.48\std{2.70} & 69.43\std{2.84} & 50.99\std{3.15} \\

1 & 10 & -0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.30 \includegraphics[width=0.8em]{pic/frozen.pdf} & 57.33\std{0.95}& 54.06\std{1.47}& 54.44\std{1.33}& 53.73\std{1.47}& 74.82\std{1.36}& 58.24\std{1.78} \\

1 & 10 & -0.25 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.40 \includegraphics[width=0.8em]{pic/frozen.pdf} & 57.08\std{1.46}& 53.31\std{0.98}& 53.24\std{1.14}& 52.87\std{0.98}& 73.77\std{1.28}& 56.86\std{1.47} \\

1 & 11 & -0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.30 \includegraphics[width=0.8em]{pic/frozen.pdf} & 56.68\std{1.30}& 53.04\std{2.00}& 53.45\std{2.03}& 52.84\std{2.30}& 73.81\std{1.55}& 57.34\std{1.46} \\

1 & 10 & -0.19 \includegraphics[width=0.8em]{pic/learnable.pdf} & -0.27 \includegraphics[width=0.8em]{pic/learnable.pdf} & \textbf{58.56\std{0.93}}& \textbf{55.65\std{0.81}}& \textbf{55.86\std{0.79}}& \textbf{55.42\std{0.82}}& \textbf{76.07\std{0.59}}& \textbf{59.75\std{0.67}} \\

1 & 7 & \;0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} & -0.60 \includegraphics[width=0.8em]{pic/learnable.pdf} & 56.36\std{0.58}& 53.91\std{1.10}& 54.34\std{1.03}& 53.78\std{0.91}& 74.19\std{0.69}& 56.62\std{1.28} \\

1 & 9 & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} & -0.60 \includegraphics[width=0.8em]{pic/learnable.pdf} & 55.20\std{1.50}& 53.05\std{1.14}& 53.21\std{1.06}& 52.76\std{1.02}& 73.09\std{1.13}& 55.50\std{1.71} \\

1 & 10 & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} & 57.11\std{0.92}& 55.04\std{1.43}& 55.53\std{1.57}& 54.58\std{1.29}& 75.13\std{1.33}& 58.47\std{1.43} \\

1 & 11 & -0.20 \includegraphics[width=0.8em]{pic/learnable.pdf} & -0.30 \includegraphics[width=0.8em]{pic/learnable.pdf} & 57.83\std{1.16}& 54.32\std{1.22}& 54.51\std{1.18}& 54.01\std{1.21}& 74.74\std{1.12}& 57.96\std{1.08} \\

1 & 11 & -0.18 \includegraphics[width=0.8em]{pic/learnable.pdf} & -0.25 \includegraphics[width=0.8em]{pic/learnable.pdf} & 57.00\std{1.32}& 53.00\std{2.28}& 53.17\std{1.94}& 52.32\std{2.19}& 73.97\std{1.89}& 57.00\std{1.93} \\

\bottomrule
\end{tabular}
}
\label{tab:ablation_ADFTD}
\end{table}



==> table/Ablation/Ablation_APAVA.tex <==

% \begin{table}[htp]
% \centering
% \caption{Ablation study of CIF structure hyperparameters on APAVA dataset (16 Channels). We use \includegraphics[width=1em]{pic/learnable.pdf} to represent learnable parameters, and \includegraphics[width=1em]{pic/frozen.pdf} to represent non-learnable parameters.}
% \begin{tabular}{cccc*{6}{>{\centering\arraybackslash}p{1.1cm}}}
% \toprule
% \multicolumn{1}{c}{\textbf{t }} & \multicolumn{1}{c}{\textbf{n }} & \multicolumn{1}{c}{\textbf{a }}  & \multicolumn{1}{c}{\textbf{b }}  &\multicolumn{1}{c}{\textbf{Accuracy \uparrow}} & \multicolumn{1}{c}{\textbf{Precision \uparrow}} & \multicolumn{1}{c}{\textbf{Recall \uparrow}} & \multicolumn{1}{c}{\textbf{F1 score \uparrow}} & \multicolumn{1}{c}{\textbf{AUROC \uparrow}} & \multicolumn{1}{c}{\textbf{AUPRC \uparrow}}  \\
% \midrule

% - & - 
% & -
% & -
% & 82.49\std{1.40} & 82.38\std{1.79} & 81.20\std{1.32} & 81.60\std{1.39} & 91.10\std{1.63} & 91.30\std{1.71} \\

% -1 & 5 
% & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 81.48\std{1.96}& 81.99\std{2.38}& 79.52\std{2.00}& 80.21\std{2.07}& 90.93\std{1.74}& 91.17\std{1.77} \\

% -1 & 6 
% & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 84.00\std{2.37}& 84.33\std{2.61}& 82.37\std{2.44}& 83.02\std{2.50}& 92.67\std{2.57}& 92.87\std{2.55} \\

% -1 &  7
% & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 81.77\std{2.31}& 82.67\std{3.24}& 79.78\std{2.04}& 80.49\std{2.26}& 89.92\std{2.60}& 90.23\std{2.53}  \\


% 1 & 9 
% & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & \textbf{85.16\std{1.55}}& \textbf{84.76\std{1.62}}& \textbf{85.33\std{1.27}}& \textbf{84.82\std{1.49}}& \textbf{94.06\std{1.07}}& \textbf{94.21\std{0.99}} \\

% -1 & 10 
% & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} 
% & 82.60\std{1.82}& 82.30\std{2.04}& 81.92\std{2.29}& 81.92\std{1.95}& 91.94\std{1.55}& 92.16\std{1.50} \\

% -1 & 11 
% & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 2 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 78.98\std{0.97}& 78.57\std{1.09}& 77.60\std{0.93}& 77.93\std{0.97}& 87.29\std{0.93}& 87.35\std{0.96}  \\

% \bottomrule
% \end{tabular}
% \label{tab:ablation}
% \end{table}

\begin{table}[htp]
\centering
\caption{Ablation study of CIF structure hyperparameters on APAVA dataset (16 Channels). We use \includegraphics[width=1em]{pic/learnable.pdf} to represent learnable parameters, and \includegraphics[width=1em]{pic/frozen.pdf} to represent non-learnable parameters.}

\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc*{6}{>{\centering\arraybackslash}p{1.1cm}}}
\toprule
\multicolumn{1}{c}{\textbf{t }} & \multicolumn{1}{c}{\textbf{n }} & \multicolumn{1}{c}{\textbf{a }}  & \multicolumn{1}{c}{\textbf{b }}  &\multicolumn{1}{c}{\textbf{Accuracy $\uparrow$}} & \multicolumn{1}{c}{\textbf{Precision $\uparrow$}} & \multicolumn{1}{c}{\textbf{Recall $\uparrow$}} & \multicolumn{1}{c}{\textbf{F1 score $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUROC $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUPRC $\uparrow$}}  \\
\midrule

- & - & - & - & 82.49\std{1.40} & 82.38\std{1.79} & 81.20\std{1.32} & 81.60\std{1.39} & 91.10\std{1.63} & 91.30\std{1.71} \\

-1 & 5 & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} & 81.48\std{1.96}& 81.99\std{2.38}& 79.52\std{2.00}& 80.21\std{2.07}& 90.93\std{1.74}& 91.17\std{1.77} \\

-1 & 6 & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} & 84.00\std{2.37}& 84.33\std{2.61}& 82.37\std{2.44}& 83.02\std{2.50}& 92.67\std{2.57}& 92.87\std{2.55} \\

-1 & 7 & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} & 81.77\std{2.31}& 82.67\std{3.24}& 79.78\std{2.04}& 80.49\std{2.26}& 89.92\std{2.60}& 90.23\std{2.53} \\

1 & 9 & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} & \textbf{85.16\std{1.55}}& \textbf{84.76\std{1.62}}& \textbf{85.33\std{1.27}}& \textbf{84.82\std{1.49}}& \textbf{94.06\std{1.07}}& \textbf{94.21\std{0.99}} \\

-1 & 10 & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} & 1 \includegraphics[width=0.8em]{pic/learnable.pdf} & 82.60\std{1.82}& 82.30\std{2.04}& 81.92\std{2.29}& 81.92\std{1.95}& 91.94\std{1.55}& 92.16\std{1.50} \\

-1 & 11 & 1 \includegraphics[width=0.8em]{pic/frozen.pdf} & 2 \includegraphics[width=0.8em]{pic/frozen.pdf} & 78.98\std{0.97}& 78.57\std{1.09}& 77.60\std{0.93}& 77.93\std{0.97}& 87.29\std{0.93}& 87.35\std{0.96} \\

\bottomrule
\end{tabular}
}
\label{tab:ablation_APAVA}
\end{table}
% The ablation study demonstrates that the hyperparameters of the CIF architecture significantly impact model performance across different datasets:

% For the APAVA dataset (16 channels), the optimal configuration employs backward feature fusion (t=-1) with 9 selected channels (n=9), where the first 7 channels are fixed with reinforcement weights (a=1, non-learnable) and the remaining channels are assigned fixed suppression weights (b=1, non-learnable). This configuration achieves superior performance with 85.16% accuracy and 94.06% AUROC.

% In contrast, the ADFTD dataset (19 channels) benefits most from forward fusion (t=1) with 10 selected channels (n=10), combined with dynamic negative suppression (a=-0.19) and positive enhancement (b=0.27), yielding 58.56% accuracy and 76.07% AUROC.

% The performance variation across APAVA, ADFTD, and PTB datasets is substantial (APAVA: 78-85% accuracy vs ADFTD: 50-58%), highlighting the importance of task-specific parameter optimization. The study reveals that:
% 1. The number of selected channels (n) and fusion direction (t) are the most critical factors
% 2. Dynamic configuration of scaling factors (a/b) can further enhance model robustness
% 3. Optimal parameter settings vary significantly depending on dataset characteristics

% These findings underscore the necessity of careful hyperparameter tuning in CIF architecture implementation, particularly with regard to channel selection and fusion strategies, to achieve optimal performance across different tasks and datasets.


==> table/Ablation/Ablation_PTB.tex <==

% \begin{table}[htp]
% \centering
% \caption{Ablation study of CIF structure hyperparameters on PTB dataset (15 Channels).We use \includegraphics[width=1em]{pic/learnable.pdf} to represent learnable parameters, and \includegraphics[width=1em]{pic/frozen.pdf} to represent non-learnable parameters.}
% \begin{tabular}{cccc*{6}{>{\centering\arraybackslash}p{1.1cm}}}
% \toprule
% $t$ & $n$ & $a$ & $b$ & Acc & Prec & Rec & F1 & AUROC & AUPRC \\
% \midrule

% - & - 
% & -
% & -
% & 81.87\std{1.87} & 86.50\std{1.24} & 73.49\std{2.90} & 75.84\std{3.20} & 94.20\std{0.29} & 93.04\std{0.45} \\
% 1 & 8 
% & 0.21 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & \textbf{88.29\std{1.45}}& \textbf{90.66\std{1.48}}& \textbf{83.21\std{2.02}}& \textbf{85.59\std{1.96}}& 94.28\std{0.93}& \textbf{93.78\std{1.11}} \\

% 1 & 8 
% & 0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 84.45\std{2.15}& 88.34\std{1.15}& 77.40\std{3.52}& 79.89\std{3.51}& 93.15\std{0.70}& 91.94\std{0.67} \\

% 1 & 9 
% & 0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 85.14\std{0.22}& 87.42\std{1.08}& 79.05\std{0.52}& 81.42\std{0.35}& 93.82\std{1.19}& 92.73\std{1.27} \\

% 1 & 10 
% & 0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 85.40\std{2.08}& 88.17\std{1.96}& 79.17\std{3.12}& 81.57\std{3.07}& \textbf{94.57\std{1.13}}& 93.53\std{1.44} \\

% 1 & 11 
% & 0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 84.47\std{0.84}& 88.02\std{0.59}& 77.50\std{1.26}& 80.10\std{1.28}& 92.77\std{0.89}& 92.02\std{0.78} \\

% 1 & 8 
% & 0.23 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 83.96\std{5.41}& 87.13\std{3.96}& 76.89\std{8.22}& 78.66\std{9.51}& 92.49\std{2.91}& 91.14\std{3.79} \\

% 1 & 8 
% & 0.25 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} 
% & 85.56\std{2.09}& 88.96\std{1.77}& 79.03\std{3.03}& 81.61\std{3.14}& 93.61\std{1.11}& 93.07\std{1.03} \\

% \bottomrule
% \end{tabular}
% \label{tab:ablation}
% \end{table}

\begin{table}[htp]
\centering
\caption{Ablation study of CIF structure hyperparameters on PTB dataset (15 Channels). We use \includegraphics[width=1em]{pic/learnable.pdf} to represent learnable parameters, and \includegraphics[width=1em]{pic/frozen.pdf} to represent non-learnable parameters.}

\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc*{6}{>{\centering\arraybackslash}p{1.1cm}}}
\toprule
\multicolumn{1}{c}{\textbf{t }} & \multicolumn{1}{c}{\textbf{n }} & \multicolumn{1}{c}{\textbf{a }}  & \multicolumn{1}{c}{\textbf{b }}  &\multicolumn{1}{c}{\textbf{Accuracy $\uparrow$}} & \multicolumn{1}{c}{\textbf{Precision $\uparrow$}} & \multicolumn{1}{c}{\textbf{Recall $\uparrow$}} & \multicolumn{1}{c}{\textbf{F1 score $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUROC $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUPRC $\uparrow$}}  \\
\midrule

- & - & - & - & 81.87\std{1.87} & 86.50\std{1.24} & 73.49\std{2.90} & 75.84\std{3.20} & 94.20\std{0.29} & 93.04\std{0.45} \\

1 & 8 & 0.21 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & \textbf{88.29\std{1.45}}& \textbf{90.66\std{1.48}}& \textbf{83.21\std{2.02}}& \textbf{85.59\std{1.96}}& 94.28\std{0.93}& \textbf{93.78\std{1.11}} \\

1 & 8 & 0.20 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & 84.45\std{2.15}& 88.34\std{1.15}& 77.40\std{3.52}& 79.89\std{3.51}& 93.15\std{0.70}& 91.94\std{0.67} \\

1 & 9 & 0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & 85.14\std{0.22}& 87.42\std{1.08}& 79.05\std{0.52}& 81.42\std{0.35}& 93.82\std{1.19}& 92.73\std{1.27} \\

1 & 10 & 0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & 85.40\std{2.08}& 88.17\std{1.96}& 79.17\std{3.12}& 81.57\std{3.07}& \textbf{94.57\std{1.13}}& 93.53\std{1.44} \\

1 & 11 & 0.22 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & 84.47\std{0.84}& 88.02\std{0.59}& 77.50\std{1.26}& 80.10\std{1.28}& 92.77\std{0.89}& 92.02\std{0.78} \\

1 & 8 & 0.23 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & 83.96\std{5.41}& 87.13\std{3.96}& 76.89\std{8.22}& 78.66\std{9.51}& 92.49\std{2.91}& 91.14\std{3.79} \\

1 & 8 & 0.25 \includegraphics[width=0.8em]{pic/frozen.pdf} & -0.50 \includegraphics[width=0.8em]{pic/frozen.pdf} & 85.56\std{2.09}& 88.96\std{1.77}& 79.03\std{3.03}& 81.61\std{3.14}& 93.61\std{1.11}& 93.07\std{1.03} \\

\bottomrule
\end{tabular}
}
\label{tab:ablation_PTB}
\end{table}


==> table/Ablation/w_CIF.tex <==
\begin{table*}[!h]
    % \vspace{-2mm}
    \centering
    \caption{Ablation studies on the effects of Difference Attention (DA) under the subject-based setup.}
    \vspace{-3mm}
    % \renewcommand{\arraystretch}{1.5}
    \scalebox{0.83}{
    \begin{tabular}{l  c |c c c c| c c c c |c c c c }
    \toprule[1.5pt]
    % \toprule
       \multicolumn{2}{c|}{Datasets}  &\multicolumn{4}{c|}{APAVA}  &\multicolumn{4}{c|}{TDBRAIN} &\multicolumn{4}{c}{PTB-XL}\\
       \cmidrule(r){1-2}\cmidrule(r){3-6}\cmidrule(r){7-10}\cmidrule(r){11-14}
       \multicolumn{2}{c|}{Metrics} &Accuracy &Precision &Recall &F1 score &Accuracy &Precision &Recall & F1 score &Accuracy &Precision &Recall & F1 score \\
    \midrule[1pt]
    \multicolumn{2}{c|}{w DA} &82.60   &87.70  &78.93  &80.25  &91.04   &91.15   &91.04   &91.04   &73.87  &66.26   &61.13 &62.54    \\
    \multicolumn{2}{c|}{w/o DA} &69.88  &69.94  &66.20  &66.38    &70.52   &70.86   &70.52  &70.40   &69.33   &60.05   & 56.07 &57.63  \\
    \midrule[1pt]
    
    \multicolumn{2}{c|}{\textcolor{red}{\textbf{Improvement}}} &\textcolor{red}{\textbf{18.20\%}}  &\textcolor{red}{\textbf{25.40\%}}  &\textcolor{red}{\textbf{19.24\%}}  &\textcolor{red}{\textbf{20.89\%}}  &\textcolor{red}{\textbf{29.10\%}}   &\textcolor{red}{\textbf{28.63\%}}   &\textcolor{red}{\textbf{29.10\%}} &\textcolor{red}{\textbf{29.31\%}}  &\textcolor{red}{\textbf{6.54\%}}   &\textcolor{red}{\textbf{10.35\%}}  &\textcolor{red}{\textbf{9.02\%}}  &\textcolor{red}{\textbf{8.52\%}}  \\
    
    \bottomrule[1.5pt]
    \end{tabular}
    }
    \label{tab:abl_differential}
    \vspace{-3mm}
\end{table*}

==> table/new_ablation.tex <==

 For models where the transferred hyperparameters from HM-BiTCN do not yield optimal results, we perform additional fine-tuning. This step investigates the adaptability of CIF-related parameters and explores how they can be optimized for other model structures.
% 变色
% \begin{table}[hp]
% \centering
% \def\arraystretch{1.0}
% \caption{\textbf{Results of Subject-Independent Setup.} Green/red cells indicate performance improvement/decline with CIF.}
% \label{tab:subject-independent}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clcccccc}
%     \toprule
%     \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
%     \midrule
%     \multirow{2}{*}
%     % {\textbf{APAVA \\(2-Classes) }} 
%     {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{APAVA} \\ (2-Classes) \\Reproduced} \end{tabular}} 
%     \rowcolors{2}{gray!10}{white}
  
%    %  & iTransformer & 74.55\std{1.66} & 74.77\std{2.10} & 71.76\std{1.72} & 72.30\std{1.79} & 85.59\std{1.55} & 84.39\std{1.57} \\
%    %  & iTransformer + CIF(HM-BiTCN) & \cellcolor{green!50}74.95\std{0.87} &  74.40\std{0.75} & \cellcolor{green!50}73.79\std{1.78} & \cellcolor{green!50}73.81\std{1.43} &  84.30\std{0.88} &  82.49\std{0.96} \\

%    %    & iTransformer + CIF(New)  &\cellcolor{green!50} 75.02\std{0.86}& 74.48\std{0.76}&\cellcolor{green!50} 73.86\std{1.74}& \cellcolor{green!50}73.89\std{1.39}& 84.19\std{0.87}& 82.35\std{0.93} \\
%    % \cline{2-8}
%     & Nonformer & 71.81\std{4.20} & 71.31\std{4.40} & 70.15\std{3.38} & 70.38\std{3.74} & 71.54\std{2.73} & 72.79\std{2.50} \\
%     & Nonformer + CIF(HM-BiTCN) & \cellcolor{green!50}71.89\std{3.81} & \cellcolor{green!50}71.80\std{4.58} &  69.44\std{3.56} &  69.74\std{3.84} &  70.55\std{2.96} &  70.78\std{4.08} \\

%      & Nonformer + CIF(New)  &\cellcolor{green!50} 78.31\std{0.45}& \cellcolor{green!50}79.86\std{1.14}&\cellcolor{green!50} 75.29\std{0.30}&\cellcolor{green!50} 76.12\std{0.33}& 69.17\std{2.00}& 70.71\std{1.64}\\
  
%     \bottomrule
% \end{tabular}
% }
% \end{table}

% 彩色

\begin{table}[h]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
    \midrule
    \multirow{6}{*}
    % {\textbf{TDBrain \\(2-Classes)}} 
    {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{TDBrain} \\ (2-Classes) \\Reproduced} \end{tabular}} 
    \rowcolors{2}{gray!10}{white}
   
    & iTransformer & 74.69\std{1.02} & 74.76\std{1.04} & 74.69\std{1.02} & 74.67\std{1.02} & 83.35\std{1.24} & 83.65\std{1.41} \\
    & iTransformer + CIF(HM-BiTCN) & 72.79\std{1.12} & 72.89\std{1.16} & 72.79\std{1.12} & 72.76\std{1.11} & 81.08\std{1.03} & 81.31\std{0.93} \\

    & iTransformer + CIF(New) &\cellcolor{green!50} 76.10\std{0.76}& \cellcolor{green!50}76.16\std{0.75}&\cellcolor{green!50} 76.10\std{0.76}& \cellcolor{green!50}76.09\std{0.76}&\cellcolor{green!50} 84.79\std{1.15}&\cellcolor{green!50} 85.13\std{1.11} \\
 \cline{2-8}
 
    & Nonformer & 88.10\std{2.39} & 88.76\std{1.74} & 88.10\std{2.39} & 88.04\std{2.47} & 96.56\std{0.91} & 96.36\std{1.21} \\
    & Nonformer + CIF(HM-BiTCN) & 88.00\std{2.06}& \cellcolor{green!50}88.91\std{1.68}& 88.00\std{2.06}& 87.92\std{2.12}& \cellcolor{green!50}97.10\std{1.10}& \cellcolor{green!50}97.17\std{1.09} \\

    & Nonformer + CIF (New)& \cellcolor{green!50}88.67\std{1.30}& \cellcolor{green!50}89.34\std{0.93}&\cellcolor{green!50} 88.67\std{1.30}&\cellcolor{green!50} 88.61\std{1.33}&\cellcolor{green!50} 96.89\std{0.31}&\cellcolor{green!50} 96.91\std{0.37}\\
    \bottomrule
\end{tabular}
}
\end{table}

\begin{table}[h]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
    \midrule
    \multirow{9}{*}
    % {\textbf{ADFTD} \\ (3-Classes)} 
        {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{ADFTD} \\ (3-Classes) \\Reproduced} \end{tabular}} 
    \rowcolors{2}{gray!10}{white}
    & Autoformer & 46.90\std{2.89} & 45.59\std{2.37} & 44.91\std{2.23} & 44.34\std{2.52} & 63.49\std{2.44} & 45.63\std{2.29} \\
    & Autoformer + CIF((HM-BiTCN)) &  45.92\std{2.78} &  44.81\std{2.44} &  44.66\std{2.25} &  44.26\std{2.38} &  62.69\std{2.21} &  44.93\std{2.68} \\

     & Autoformer + CIF(New) &\cellcolor{green!50} 48.49\std{1.31}& \cellcolor{green!50}46.42\std{1.07}&\cellcolor{green!50} 45.39\std{1.80}&\cellcolor{green!50} 44.94\std{1.97}& \cellcolor{green!50}63.75\std{1.46}&\cellcolor{green!50} 46.10\std{1.84} \\
  \cline{2-8}
%     & Informer & 48.42\std{1.99} & 46.94\std{1.60} & 46.41\std{0.99} & 45.76\std{0.43} & 65.99\std{1.14} & 47.49\std{1.07} \\
%     & Informer + CIC(HM-BiTCN) & \cellcolor{green!50}50.12\std{0.66} & \cellcolor{green!50}47.23\std{0.47} & \cellcolor{green!50}46.77\std{0.39} & \cellcolor{green!50}46.62\std{0.38} &  65.13\std{0.52} &  46.84\std{0.54} \\

    
% \cline{2-8}
    
    & iTransformer & 52.85\std{1.36} & 46.97\std{1.05} & 47.31\std{1.03} & 46.84\std{0.78} & 67.46\std{0.96} & 49.90\std{0.89} \\
    & iTransformer + CIF(HM-BiTCN) &  50.76\std{0.50} & \cellcolor{green!50}47.11\std{0.67} &  47.29\std{0.59} & \cellcolor{green!50}47.10\std{0.66} &  67.00\std{0.55} &  49.60\std{0.69} \\
    & iTransformer + CIF(New) & \cellcolor{green!50}53.93\std{1.52}& \cellcolor{green!50}48.44\std{0.89}&\cellcolor{green!50} 49.13\std{1.17}&\cellcolor{green!50} 48.56\std{0.84}&\cellcolor{green!50} 68.70\std{0.94}&\cellcolor{green!50} 50.88\std{1.20} \\
   \cline{2-8}
    & Reformer & 51.28\std{2.60} & 49.68\std{2.75} & 49.64\std{2.02} & 48.45\std{2.06} & 69.20\std{2.53} & 51.74\std{3.24} \\
    & Reformer + CIF(HM-BiTCN) & \cellcolor{green!50}52.50\std{0.91} & \cellcolor{green!50}52.10\std{2.91} &  49.01\std{2.74} &  47.53\std{4.23} &  68.25\std{1.79} &  50.44\std{2.59} \\

   & Reformer + CIF(New) & \cellcolor{green!50}53.11\std{1.71}& \cellcolor{green!50}52.14\std{1.42}& \cellcolor{green!50}52.42\std{1.90}& \cellcolor{green!50}51.73\std{2.01}& \cellcolor{green!50}70.47\std{1.64}& \cellcolor{green!50}51.88\std{1.92}  \\
  \cline{2-8}
    & Medformer & 53.70\std{1.18} & 51.51\std{1.32} & 50.49\std{1.48} & 50.35\std{1.53} & 70.48\std{1.17} & 50.91\std{1.13} \\
    & Medformer + CIF(HM-BiTCN) & \cellcolor{green!50}55.88\std{0.82} & \cellcolor{green!50}51.91\std{1.90} & \cellcolor{green!50}50.80\std{1.63} &  50.29\std{1.92} &  70.45\std{1.33} & \cellcolor{green!50}53.73\std{1.70} \\

    & Medformer + CIF(New) & \cellcolor{green!50}55.21\std{1.42}& \cellcolor{green!50}52.84\std{2.36}& \cellcolor{green!50}52.60\std{2.26}& \cellcolor{green!50}52.43\std{2.65}& \cellcolor{green!50}72.11\std{2.42}& \cellcolor{green!50}54.10\std{3.09}\\
   
    \bottomrule
\end{tabular}
}
\end{table}

% 变色





\begin{table}[h]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
    \midrule
    \multirow{8}{*}
    % {\textbf{APAVA \\(2-Classes) }} 
    {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB} \\ (2-Classes) \\Reproduced} \end{tabular}} 
    \rowcolors{2}{gray!10}{white}
  
    & iTransformer & 83.43\std{1.19} & 88.06\std{1.47} & 75.64\std{1.55} & 78.29\std{1.70} & 91.38\std{1.41} & 91.08\std{1.30}  \\
    & iTransformer + CIF(HM-BiTCN) &  81.62\std{2.96} &  87.48\std{2.03} &  72.74\std{4.41} &  74.99\std{4.91} &  90.25\std{3.29} &  89.80\std{3.28} \\

     & iTransformer + CIF(New) & \cellcolor{green!50}83.56\std{1.15}& 86.00\std{1.03}& \cellcolor{green!50}76.78\std{1.94}&\cellcolor{green!50} 79.10\std{1.87}& 90.40\std{0.75}& 89.80\std{0.93} \\
    
   \cline{2-8}
    & Nonformer & 78.93\std{1.46} & 82.48\std{1.53} & 69.68\std{2.15} & 71.50\std{2.56} & 90.54\std{0.59} & 87.78\std{1.46}  \\
    & Nonformer + CIF(HM-BiTCN) &  71.89\std{3.81} &  71.80\std{4.58} &  69.44\std{3.56} &  69.74\std{3.84} &  70.55\std{2.96} &  70.78\std{4.08} \\

   & Nonformer + CIF(New) &\cellcolor{green!50} 80.46\std{2.20}& \cellcolor{green!50}84.22\std{2.44}&\cellcolor{green!50} 71.79\std{3.10}&\cellcolor{green!50} 73.89\std{3.50}&\cellcolor{green!50} 92.74\std{0.97}&\cellcolor{green!50} 90.30\std{1.26}\\
    \cline{2-8}
   
    & Medformer  & 80.99\std{0.75} & 83.01\std{0.72} & 73.35\std{1.16} & 75.47\std{1.21} & 93.10\std{1.18} & 90.69\std{1.04} \\
    & Medformer + CIF(HM-BiTCN) &  78.74\std{0.64} & 81.11\std{0.84} & \cellcolor{green!50}75.40\std{0.66} & \cellcolor{green!50}76.31\std{0.71} &  83.20\std{0.91} &  83.66\std{0.92} \\
    
   & Medformer + CIF(New)& \cellcolor{green!50}83.98\std{0.81}& \cellcolor{green!50}85.21\std{0.62}& \cellcolor{green!50}78.00\std{1.30}& \cellcolor{green!50}80.11\std{1.22}& \cellcolor{green!50}93.32\std{0.97}& \cellcolor{green!50}90.97\std{1.69} \\
  
    \bottomrule
\end{tabular}
}
\end{table}



% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%        \includegraphics[width=\linewidth]{pic/APAVA+CIF.pdf}
%         \caption{APAVA}  % 自动显示 (a)
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/TDBrain+CIF.pdf}
%         \caption{TDBRAIN}  % 自动显示 (b)
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/PTB+CIF.pdf}
%         \caption{PTB}  % 自动显示 (b)ADFTD
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.24\textwidth}
%         \centering
%           \includegraphics[width=\linewidth]{pic/ADFTD+CIF.pdf}
%         \caption{ADFTD}  % 自动显示 (b)
%     \end{subfigure}
%     \caption{The improvements achieved by various baselines when combined with the CIF method.} 
%         \label{fig_APAVA_TDBrain_PTB_APAVA}
% \end{figure}



% \begin{figure}[ht]
%     \centering
    % \begin{subfigure}{0.48\textwidth}
    %     \centering
    %    \includegraphics[width=\linewidth]{pic/柱状图_APAVA.pdf}
    %     \caption{APAVA}  % 自动显示 (a)
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\textwidth}
    %     \centering
    %       \includegraphics[width=\linewidth]{pic/柱状图TDBrain.pdf}
    %     \caption{TDBRAIN}  % 自动显示 (b)
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\textwidth}
    %     \centering
    %       \includegraphics[width=\linewidth]{pic/柱状图PTB.pdf}
    %     \caption{PTB}  % 自动显示 (b)ADFTD
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\textwidth}
    %     \centering
    %       \includegraphics[width=\linewidth]{pic/柱状图ADFTD.pdf}
    %     \caption{ADFTD}  % 自动显示 (b)
    % \end{subfigure}
%     \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{pic/柱状图_APAVA.pdf}
%     \caption{Performance improvement on the APAVA dataset using the CIF method.}
%     \label{fig:apava}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{pic/柱状图TDBrain.pdf}
%     \caption{Performance improvement on the TDBRAIN dataset using the CIF method.}
%     \label{fig:tdbrain}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{pic/柱状图PTB.pdf}
%     \caption{Performance improvement on the PTB dataset using the CIF method.}
%     \label{fig:ptb}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\linewidth]{pic/柱状图ADFTD.pdf}
%     \caption{Performance improvement on the ADFTD dataset using the CIF method.}
%     \label{fig:adftd}
% \end{figure}

%     \caption{The improvements achieved by various baselines when combined with the CIF method.} 
%         \label{fig_APAVA_TDBrain_PTB_APAVA}
% \end{figure}




% \begin{table}[h]
% \centering
% \def\arraystretch{1.0}
% \caption{\textbf{Results of Subject-Independent Setup.} Green/red cells indicate performance improvement/decline with CIF.}
% \label{tab:subject-independent}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clcccccc}
%     \toprule
%     \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPRC}}  \\
%     \midrule
%     \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB} \\ (2-Classes)} \end{tabular}} 
%     \rowcolors{2}{gray!10}{white} % Set row colors (alternating gray and white)
  
%     & iTransformer & 83.43\std{1.19} & 88.06\std{1.47} & 75.64\std{1.55} & 78.29\std{1.70} & 91.38\std{1.41} & 91.08\std{1.30}  \\
%     & iTransformer + CIF(HM-BiTCN) &  81.62\std{2.96} &  87.48\std{2.03} &  72.74\std{4.41} &  74.99\std{4.91} &  90.25\std{3.29} &  89.80\std{3.28} \\

%      & iTransformer + CIF(New) & \cellcolor{green!50}83.56\std{1.15}& 86.00\std{1.03}& \cellcolor{green!50}76.78\std{1.94}&\cellcolor{green!50} 79.10\std{1.87}& 90.40\std{0.75}& 89.80\std{0.93} \\
    
%    \cline{2-8}
%     & Nonformer & 78.93\std{1.46} & 82.48\std{1.53} & 69.68\std{2.15} & 71.50\std{2.56} & 90.54\std{0.59} & 87.78\std{1.46}  \\
%     & Nonformer + CIF(HM-BiTCN) &  71.89\std{3.81} &  71.80\std{4.58} &  69.44\std{3.56} &  69.74\std{3.84} &  70.55\std{2.96} &  70.78\std{4.08} \\

%    & Nonformer + CIF(New) &\cellcolor{green!50} 80.46\std{2.20}& \cellcolor{green!50}84.22\std{2.44}&\cellcolor{green!50} 71.79\std{3.10}&\cellcolor{green!50} 73.89\std{3.50}&\cellcolor{green!50} 92.74\std{0.97}&\cellcolor{green!50} 90.30\std{1.26}\\
%     \cline{2-8}
   
%     & Medformer  & 80.99\std{0.75} & 83.01\std{0.72} & 73.35\std{1.16} & 75.47\std{1.21} & 93.10\std{1.18} & 90.69\std{1.04} \\
%     & Medformer + CIF(HM-BiTCN) &  78.74\std{0.64} & \cellcolor{green!50}81.11\std{0.84} & \cellcolor{green!50}75.40\std{0.66} & \cellcolor{green!50}76.31\std{0.71} &  83.20\std{0.91} &  83.66\std{0.92} \\
    
%    & Medformer + CIF(New)& \cellcolor{green!50}83.98\std{0.81}& \cellcolor{green!50}85.21\std{0.62}& \cellcolor{green!50}78.00\std{1.30}& \cellcolor{green!50}80.11\std{1.22}& \cellcolor{green!50}93.32\std{0.97}& \cellcolor{green!50}90.97\std{1.69} \\
%     \bottomrule
% \end{tabular}
% }
% \end{table}

% \end{document}


==> table/process_dataset.tex <==




\begin{table}[!htbp]
    \centering
    \scriptsize
    \caption{\textbf{The information of processed datasets.} The table shows the number of subjects, samples, classes, channels, sampling rate, sample timestamps, modality of MedTS, and file size. Here, \textbf{\#-Timestamps} indicates the number of timestamps per sample.All data processing procedures follow those of Medformer~\cite{wang2024medformer}.
    }
    % \vspace{-3mm}
    \label{tab:processed_data}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}ll|cccccccc@{}}
    \toprule
    \multicolumn{2}{l|}{Datasets} & \#-Subject & \#-Sample & \#-Class & \#-Channel & \#-Timestamps & Sampling Rate & Modality & File Size  \\ \midrule
    \multicolumn{2}{l|}{APAVA} &  23     & 5,967 &  2  & 16 & 256 &  256Hz  & EEG & 186MB \\
    \multicolumn{2}{l|}{ADFTD} &  88  & 69,752 &  3  & 19 & 256 &  256Hz  & EEG & 2.52GB \\
    \multicolumn{2}{l|}{TDBrain} &  72  & 6,240 &  2  & 33 & 256 &  256Hz  & EEG & 571MB \\
    \multicolumn{2}{l|}{PTB} &  198  & 64,356 &  2  & 15 & 300 &  250Hz  & ECG & 2.15GB \\
    \multicolumn{2}{l|}{PTB-XL} &  17,596  & 191,400 &  5  & 12 & 250 &  250Hz  & ECG & 4.28GB \\
    % \multicolumn{2}{l|}{EEGMMIDB} &  106  & 9236 &  3  & 64 & 640 &  160Hz  & Type-II & 2.82GB \\
    % \multicolumn{2}{l|}{WG-fNIRS} &  26  & 9360 &  2  & 72 & 25 &  10Hz  & Type-II & 129MB \\
    \bottomrule
    \end{tabular}
    } % End of first resizebox
    % \vspace{-8mm}
\end{table}


\begin{table}[thbp]
    \centering
    \caption{Datasets and mapping details of UEA dataset \citep{bagnall2018uea}.}
      % \vskip 0.1in
    \label{tab:uea_datasets}
    \begin{tabular}{|l|c c | c | c|}
        \hline
        Dataset & Sample Numbers(train set,test set) & Variable Number & Series Length \\
        \hline
        EthanolConcentration & (261, 263) & 3 & 1751 \\
        FaceDetection & (5890, 3524) & 144 & 62 \\
        Handwriting & (150, 850) & 3 & 152 \\
        Heartbeat & (204, 205) & 61 & 405 \\
        JapaneseVowels & (270, 370) & 12 & 29 \\
        PEMSSF & (267, 173) & 963 & 144 \\
        SelfRegulationSCP1 & (268, 293) & 6 & 896 \\
        SelfRegulationSCP2 & (200, 180) & 7 & 1152 \\
        SpokenArabicDigits & (6599, 2199) & 13 & 93 \\
        UWaveGestureLibrary & (120, 320) & 3 & 315 \\
        \hline
    \end{tabular}
\end{table}

==> table/produce_score.tex <==
\begin{table}
\centering
% \scriptsize
\def\arraystretch{0.95}
\caption{
\textbf{
Results of Subject-Independent Setup.} The training, validation, and test sets are distributed based on subjects according to a predetermined ratio/IDs. Results of the APAVA, TDBrain, ADFTD, PTB, and PTB-XL datasets under this setup are presented here. Unfortunately, MedGNN has only released the training parameters for the APAVA and ADFTD datasets.
}
\label{tab:subject-independent-reproduce}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    % \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy \uparrow}} & \multicolumn{1}{c}{\textbf{Precision \uparrow}} & \multicolumn{1}{c}{\textbf{Recall \uparrow}} & \multicolumn{1}{c}{\textbf{F1 score \uparrow}} & \multicolumn{1}{c}{\textbf{AUROC \uparrow}} & \multicolumn{1}{c}{\textbf{AUPRC \uparrow}}  \\
      \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy $\uparrow$}} & \multicolumn{1}{c}{\textbf{Precision $\uparrow$}} & \multicolumn{1}{c}{\textbf{Recall $\uparrow$}} & \multicolumn{1}{c}{\textbf{F1 score $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUROC $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUPRC $\uparrow$}} \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{APAVA} \\ (2-Classes) \\Reproduced} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer}& 73.18\std{7.33}& 73.87\std{6.72}& 73.01\std{6.10}& 72.40\std{7.03}& 81.64\std{7.24}& 81.10\std{7.75}\\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 72.76\std{2.04}& 79.64\std{2.45}& 67.41\std{2.62}& 66.88\std{3.61}& 71.81\std{4.06}& 71.64\std{3.74}  \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 75.16\std{1.67}& 74.98\std{0.69}& 73.34\std{2.97}& 73.50\std{2.90}& 83.89\std{1.54}& 83.27\std{1.62}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 72.20\std{2.78}& 73.92\std{4.80}& 68.48\std{2.51}& 68.74\std{2.70}& 70.14\std{3.43}& 70.84\std{3.80}   \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 74.55\std{1.66}& 74.77\std{2.10}& 71.76\std{1.72}& 72.30\std{1.79}& 85.59\std{1.55}& 84.39\std{1.57}  \\
    & \textbf{MTST}~\cite{zhang2024multi} & 69.24\std{1.24}& 75.87\std{2.80}& 63.28\std{1.81}& 61.62\std{2.75}& 66.09\std{3.27}& 68.08\std{2.93} \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 71.81\std{4.20}& 71.31\std{4.40}& 70.15\std{3.38}& 70.38\std{3.74}& 71.54\std{2.73}& 72.79\std{2.50} \\
    & \textbf{PatchTST}~\cite{nie2022time} & 68.27\std{2.11}& 78.56\std{1.88}& 61.53\std{2.60}& 58.52\std{4.07}& 64.61\std{2.18}& 67.14\std{2.06}  \\
    & \textbf{Reformer}~\cite{kitaev2019reformer} & 78.42\std{2.85}& 80.89\std{4.52}& 75.20\std{2.28}& 76.09\std{2.54}& 75.48\std{2.79}& 77.52\std{2.64} \\
    & \textbf{Transformer}~\cite{vaswani2017attention} & 75.53\std{4.28}& 76.90\std{5.05}& 72.14\std{4.87}& 72.64\std{5.44}& 72.30\std{6.04}& 73.04\std{7.15}\\

    & \textbf{Medformer}~\cite{wang2024medformer} & 77.85\std{2.42}& 80.31\std{3.21}& 74.38\std{2.49}& 75.21\std{2.67}& 80.85\std{3.80}& 81.62\std{3.24}  \\

     & \textbf{MedGNN}~\cite{fan2025medgnn}  & 77.40\std{5.77}& 82.77\std{4.46}& 73.24\std{7.06}& 73.29\std{9.01}& 81.31\std{2.94}& 82.80\std{2.91}   \\
     & \textbf{HM-BiTCN + CIF} & \textbf{85.16\std{1.55}} & \textbf{84.76\std{1.62}} & \textbf{85.33\std{1.27}} & \textbf{84.82\std{1.49}} & \textbf{94.06\std{1.07}} & \textbf{94.21\std{0.99}}  \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{TDBrain} \\ (2-Classes) \\Reproduced} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 90.38\std{3.03}& 91.16\std{2.42}& 90.38\std{3.03}& 90.31\std{3.09}& 95.83\std{2.14}& 95.43\std{2.31} \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 82.15\std{2.60}& 82.81\std{2.11}& 82.15\std{2.60}& 82.04\std{2.70}& 91.20\std{2.23}& 91.47\std{2.16} \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 77.60\std{1.23}& 78.25\std{1.52}& 77.60\std{1.23}& 77.48\std{1.19}& 86.31\std{1.23}& 86.48\std{1.36}\\
    & \textbf{Informer}~\cite{zhou2021informer} & 88.42\std{2.99}& 89.01\std{2.45}& 88.42\std{2.99}& 88.36\std{3.05}& 96.54\std{0.90}& 96.66\std{0.85}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 74.69\std{1.02}& 74.76\std{1.04}& 74.69\std{1.02}& 74.67\std{1.02}& 83.35\std{1.24}& 83.65\std{1.41}  \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 77.67\std{3.58}& 78.97\std{4.37}& 77.67\std{3.58}& 77.45\std{3.55}& 86.47\std{4.84}& 84.99\std{6.43}  \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 88.10\std{2.39}& 88.76\std{1.74}& 88.10\std{2.39}& 88.04\std{2.47}& 96.56\std{0.91}& 96.36\std{1.21}  \\
    & \textbf{PatchTST}~\cite{nie2022time}  & 77.98\std{2.64}& 79.30\std{3.73}& 77.98\std{2.64}& 77.76\std{2.65}& 86.67\std{4.03}& 84.93\std{5.47} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 88.50\std{2.30}& 89.01\std{1.80}& 88.50\std{2.30}& 88.45\std{2.35}& 96.10\std{0.63}& 96.19\std{0.55} \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 85.13\std{1.86}& 86.39\std{1.56}& 85.13\std{1.86}& 84.99\std{1.93}& 95.61\std{1.05}& 95.63\std{0.91} \\
    & \textbf{Medformer}~\cite{wang2024medformer}  & 88.77\std{1.24}& 88.91\std{1.11}& 88.77\std{1.24}& 88.76\std{1.25}& 96.38\std{0.34}& 96.44\std{0.30} \\
     & \textbf{MedGNN}~\cite{fan2025medgnn}  & - & - & - & - & - & -  \\
     % & \textbf{HM-BiTCN(Ours)}  & \textbf{93.17\std{1.33}} & \textbf{93.44\std{1.18}} & \textbf{93.17\std{1.33}} & \textbf{93.15\std{1.34}} & \textbf{98.73\std{0.53}} & \textbf{98.77\std{0.51}} & 0.00\std{0.00} \\
     & \textbf{HM-BiTCN + CIF}  & \textbf{93.13\std{1.41}} & \textbf{93.33\std{1.37}} & \textbf{93.13\std{1.41}} & \textbf{93.12\std{1.42}} & \textbf{98.62\std{0.66}} & \textbf{98.68\std{0.63}}  \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{ADFTD} \\ (3-Classes) \\Reproduced} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 46.90\std{2.89}& 45.59\std{2.37}& 44.91\std{2.23}& 44.34\std{2.52}& 63.49\std{2.44}& 45.63\std{2.29} \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 50.18\std{1.97}& 45.97\std{1.84}& 46.30\std{1.73}& 45.90\std{1.84}& 66.68\std{1.67}& 48.65\std{1.89} \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 45.75\std{0.78}& 45.71\std{1.29}& 44.27\std{1.28}& 43.51\std{1.00}& 62.64\std{1.64}& 45.88\std{1.35}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 48.42\std{1.99}& 46.94\std{1.60}& 46.41\std{0.99}& 45.76\std{0.43}& 65.99\std{1.14}& 47.49\std{1.07}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 52.85\std{1.36}& 46.97\std{1.05}& 47.31\std{1.03}& 46.84\std{0.78}& 67.46\std{0.96}& 49.90\std{0.89}  \\
    & \textbf{MTST}~\cite{zhang2024multi} & 45.77\std{1.70}& 44.39\std{1.73}& 43.70\std{1.82}& 43.36\std{1.98}& 61.38\std{1.57}& 44.01\std{1.60}  \\
    & \textbf{Nonformer}~\cite{liu2022non}   & 50.81\std{1.06}& 48.71\std{1.40}& 48.55\std{1.47}& 48.36\std{1.38}& 66.95\std{1.54}& 48.08\std{1.82} \\
    & \textbf{PatchTST}~\cite{nie2022time}  & 43.32\std{0.53}& 41.95\std{0.38}& 41.45\std{1.26}& 40.75\std{1.62}& 60.21\std{0.29}& 42.49\std{0.57} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 51.28\std{2.60}& 49.68\std{2.75}& 49.64\std{2.02}& 48.45\std{2.06}& 69.20\std{2.53}& 51.74\std{3.24}  \\
    & \textbf{Transformer}~\cite{vaswani2017attention}   & 50.53\std{0.94}& 49.31\std{0.87}& 48.57\std{1.23}& 48.42\std{1.28}& 67.98\std{0.90}& 49.07\std{1.35} \\
    & \textbf{Medformer}~\cite{wang2024medformer} & 53.70\std{1.18}& 51.51\std{1.32}& 50.49\std{1.48}& 50.35\std{1.53}& 70.48\std{1.17}& 50.91\std{1.13} \\
    & \textbf{MedGNN}~\cite{fan2025medgnn}  & 50.22\std{3.21}& 48.65\std{3.72}& 47.50\std{4.57}& 47.33\std{4.40}& 67.18\std{4.39}& 48.84\std{4.11}  \\
 
      & \textbf{HM-BiTCN + CIF}  & \textbf{58.56\std{0.93}} & \textbf{55.65\std{0.81}} & \textbf{55.86\std{0.79}} & \textbf{55.42\std{0.82}} & \textbf{76.07\std{0.59}} & \textbf{59.75\std{0.67}}  \\
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB} \\ (2-Classes) \\Reproduced} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 71.99\std{2.74}& 69.60\std{3.85}& 61.50\std{4.23}& 61.43\std{5.07}& 74.29\std{1.89}& 70.26\std{2.00} \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 78.06\std{3.44}& 81.53\std{3.13}& 68.62\std{5.63}& 69.76\std{6.53}& 88.31\std{2.07}& 85.81\std{2.43}  \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 74.54\std{2.27}& 77.99\std{4.10}& 63.14\std{3.29}& 63.28\std{4.36}& 84.63\std{4.27}& 80.91\std{5.55} \\
    & \textbf{Informer}~\cite{zhou2021informer}& 79.59\std{0.65}& 83.33\std{0.77}& 70.58\std{0.95}& 72.58\std{1.08}& 92.77\std{0.48}& 90.89\std{0.57} \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 83.43\std{1.19}& 88.06\std{1.47}& 75.64\std{1.55}& 78.29\std{1.70}& 91.38\std{1.41}& 91.08\std{1.30}  \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 75.53\std{2.45}& 78.72\std{1.87}& 64.78\std{4.06}& 65.30\std{4.81}& 87.76\std{4.09}& 83.60\std{3.92} \\
    & \textbf{Nonformer}~\cite{liu2022non}  & 78.93\std{1.46}& 82.48\std{1.53}& 69.68\std{2.15}& 71.50\std{2.56}& 90.54\std{0.59}& 87.78\std{1.46} \\
    & \textbf{PatchTST}~\cite{nie2022time}  & 75.28\std{2.44}& 77.05\std{2.44}& 64.86\std{4.05}& 65.41\std{5.28}& 88.11\std{2.59}& 82.65\std{2.87} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 78.11\std{1.65}& 82.70\std{0.80}& 68.17\std{2.68}& 69.68\std{3.34}& 90.77\std{1.56}& 88.14\std{1.20}  \\
    & \textbf{Transformer}~\cite{vaswani2017attention}  & 76.43\std{1.98}& 81.25\std{1.15}& 65.64\std{3.29}& 66.44\std{4.39}& 90.21\std{1.24}& 87.28\std{1.49}  \\
    & \textbf{Medformer}~\cite{wang2024medformer}  & 80.99\std{0.75}& 83.01\std{0.72}& 73.35\std{1.16}& 75.47\std{1.21}& 93.10\std{1.18}& 90.69\std{1.04}  \\
     & \textbf{MedGNN}~\cite{fan2025medgnn}  & - & - & - & - & - & - \\
     % & \textbf{HM-BiTCN (Ours)}  & \textbf{86.77\std{1.23}} & \textbf{88.90\std{1.61}} & \textbf{81.32\std{1.64}} & \textbf{83.65\std{1.61}} & \textbf{95.15\std{0.77}} & \textbf{93.96\std{1.30}} & \textbf{0.67\std{0.09}} \\
     & \textbf{HM-BiTCN + CIF}  & \textbf{88.29\std{1.45}} & \textbf{90.66\std{1.48}} & \textbf{83.21\std{2.02}} & \textbf{85.59\std{1.96}} & \textbf{94.28\std{0.93}} & \textbf{93.78\std{1.11}}  \\

     
    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB-XL} \\ (5-Classes) \\ Reproduced} \end{tabular}} %&
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 60.37\std{1.72}& 49.83\std{0.50}& 49.17\std{0.72}& 48.43\std{0.47}& 81.35\std{0.56}& 50.83\std{0.72}  \\
    & \textbf{Crossformer}~\cite{zhang2022crossformer} & 73.15\std{0.17}& 64.62\std{0.31}& \textbf{61.28\std{0.45}}& \textbf{62.49\std{0.34}}& 89.94\std{0.15}& 67.14\std{0.29}  \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 56.01\std{10.27}& 51.61\std{5.58}& 48.77\std{7.64}& 47.23\std{8.76}& 82.01\std{4.20}& 52.23\std{7.14}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 71.28\std{0.27}& 62.28\std{0.53}& 59.18\std{0.54}& 60.38\std{0.38}& 88.57\std{0.09}& 64.57\std{0.18}  \\
    & \textbf{iTransformer}~\cite{liu2023itransformer}  & 69.18\std{0.33}& 59.44\std{0.48}& 54.84\std{0.25}& 56.44\std{0.23}& 86.65\std{0.17}& 60.27\std{0.44} \\
    & \textbf{MTST}~\cite{zhang2024multi}  & 72.14\std{0.29}& 64.01\std{0.61}& 59.31\std{0.27}& 61.07\std{0.32}& 88.82\std{0.19}& 65.52\std{0.52}  \\
    & \textbf{Nonformer}~\cite{liu2022non} & 70.51\std{0.79}& 61.42\std{1.03}& 58.15\std{0.57}& 59.31\std{0.63}& 88.20\std{0.43}& 63.33\std{0.77}  \\
    & \textbf{PatchTST}~\cite{nie2022time}  & 73.13\std{0.20}& 65.38\std{0.54}& 60.61\std{0.56}& 62.39\std{0.27}& 89.66\std{0.16}& 66.97\std{0.24}  \\
    & \textbf{Reformer}~\cite{kitaev2019reformer}  & 71.24\std{0.46}& 61.78\std{0.79}& 59.67\std{0.99}& 60.51\std{0.65}& 88.67\std{0.21}& 64.29\std{0.29}  \\
    & \textbf{Transformer}~\cite{vaswani2017attention} & 70.46\std{0.42}& 61.56\std{0.58}& 57.86\std{0.65}& 59.16\std{0.46}& 88.18\std{0.14}& 63.25\std{0.27}  \\
    & \textbf{Medformer}~\cite{wang2024medformer} & 72.94\std{0.15}& 64.39\std{0.32}& 59.98\std{0.49}& 61.61\std{0.33}& 89.67\std{0.10}& 66.25\std{0.25}  \\
    & \textbf{MedGNN}~\cite{fan2025medgnn} & - & - & - & - & - & - \\
     % & \textbf{HM-BiTCN + CIF}  & \textbf{73.32\std{1.06}} & 64.81\std{1.93} & 61.12\std{0.60} & 62.01\std{0.84} & \textbf{90.25\std{0.75}} & \textbf{67.31\std{1.55}} \\
     & \textbf{HM-BiTCN + CIF}  & \textbf{73.73\std{0.30}}&  \textbf{65.41\std{0.67}}& 60.70\std{1.08}& 61.89\std{0.91}&  \textbf{90.53\std{0.22}}&  \textbf{67.75\std{0.75}} \\
      
      
    \bottomrule
\end{tabular}
}
\end{table}

==> table/sub_CIC.tex <==


% 变色
\begin{table}[htp]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent-APAVA}
\resizebox{\textwidth}{!}{%
    \begin{tabular}{clcccccc}
        \toprule
        \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
        \midrule
        \multirow{26}{*}
        % {\textbf{APAVA \\(2-Classes) }} 
        {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{APAVA} \\ (2-Classes) \\Reproduced} \end{tabular}} 
        \rowcolors{2}{gray!10}{white}
        & Autoformer & 73.18\std{7.33} & 73.87\std{6.72} & 73.01\std{6.10} & 72.40\std{7.03} & 81.64\std{7.24} & 81.10\std{7.75} \\
        & Autoformer + CIF & \cellcolor{green!50}75.96\std{2.68} & \cellcolor{green!50}76.33\std{3.47} & \cellcolor{green!50}75.11\std{1.10} & \cellcolor{green!50}74.97\std{1.90} & \cellcolor{green!50}83.42\std{1.99} & \cellcolor{green!50}83.15\std{2.63} \\
        & Crossformer & 72.76\std{2.04} & 79.64\std{2.45} & 67.41\std{2.62} & 66.88\std{3.61} & 71.81\std{4.06} & 71.64\std{3.74} \\
        & Crossformer + CIF & \cellcolor{green!50}82.32\std{2.60} & \cellcolor{green!50}85.35\std{1.83} & \cellcolor{green!50}79.21\std{3.17} & \cellcolor{green!50}80.29\std{3.30} & \cellcolor{green!50}90.39\std{1.58} & \cellcolor{green!50}90.02\std{1.47} \\
        & FEDformer & 75.16\std{1.67} & 74.98\std{0.69} & 73.34\std{2.97} & 73.50\std{2.90} & 83.89\std{1.54} & 83.27\std{1.62} \\
        & FEDformer + CIF & \cellcolor{green!50}77.20\std{2.17} & \cellcolor{green!50}76.97\std{2.07} & \cellcolor{green!50}77.02\std{2.60} & \cellcolor{green!50}76.55\std{2.40} & \cellcolor{green!50}86.70\std{1.73} & \cellcolor{green!50}86.53\std{1.76} \\
        & Informer & 72.20\std{2.78} & 73.92\std{4.80} & 68.48\std{2.51} & 68.74\std{2.70} & 70.14\std{3.43} & 70.84\std{3.80} \\
        & Informer + CIF & \cellcolor{green!50}79.78\std{2.07} & \cellcolor{green!50}82.29\std{3.03} & \cellcolor{green!50}76.55\std{2.05} & \cellcolor{green!50}77.53\std{2.23} & \cellcolor{green!50}78.56\std{1.33} & \cellcolor{green!50}78.58\std{1.14} \\
        & iTransformer & 74.55\std{1.66} & 74.77\std{2.10} & 71.76\std{1.72} & 72.30\std{1.79} & 85.59\std{1.55} & 84.39\std{1.57} \\
        & iTransformer + CIF & \cellcolor{green!50}74.95\std{0.87} & 74.40\std{0.75} & \cellcolor{green!50}73.79\std{1.78} & \cellcolor{green!50}73.81\std{1.43} & 84.30\std{0.88} & 82.49\std{0.96} \\
        & MTST & 69.24\std{1.24} & 75.87\std{2.80} & 63.28\std{1.81} & 61.62\std{2.75} & 66.09\std{3.27} & 68.08\std{2.93} \\
        & MTST + CIF & \cellcolor{green!50}76.20\std{2.39} & \cellcolor{green!50}81.46\std{1.11} & \cellcolor{green!50}71.67\std{3.06} & \cellcolor{green!50}72.06\std{3.73} & \cellcolor{green!50}77.65\std{3.37} & \cellcolor{green!50}77.98\std{2.73} \\
        & Nonformer & 71.81\std{4.20} & 71.31\std{4.40} & 70.15\std{3.38} & 70.38\std{3.74} & 71.54\std{2.73} & 72.79\std{2.50} \\
        & Nonformer + CIF & \cellcolor{green!50}71.89\std{3.81} & \cellcolor{green!50}71.80\std{4.58} & 69.44\std{3.56} &69.74\std{3.84} & 70.55\std{2.96} & 70.78\std{4.08} \\
        & Reformer & 78.42\std{2.85} & 80.89\std{4.52} & 75.20\std{2.28} & 76.09\std{2.54} & 75.48\std{2.79} & 77.52\std{2.64} \\
        & Reformer + CIF & \cellcolor{green!50}81.51\std{0.57} & \cellcolor{green!50}\textbf{84.90\std{0.86}} & \cellcolor{green!50}78.18\std{0.60} & \cellcolor{green!50}79.32\std{0.64} & \cellcolor{green!50}79.10\std{2.50} & \cellcolor{green!50}80.77\std{2.21} \\
        & Transformer & 75.53\std{4.28} & 76.90\std{5.05} & 72.14\std{4.87} & 72.64\std{5.44} & 72.30\std{6.04} & 73.04\std{7.15} \\
        & Transformer + CIF & \cellcolor{green!50}77.96\std{2.82} & \cellcolor{green!50}79.34\std{3.86} & \cellcolor{green!50}75.07\std{2.52} & \cellcolor{green!50}75.87\std{2.73} & \cellcolor{green!50}74.75\std{1.62} & \cellcolor{green!50}74.76\std{2.33} \\
        & Medformer & 77.85\std{2.42} & 80.31\std{3.21} & 74.38\std{2.49} & 75.21\std{2.67} & 80.85\std{3.80} & 81.62\std{3.24} \\
        & Medformer + CIF & \cellcolor{green!50}81.06\std{1.58} & \cellcolor{green!50}82.97\std{2.23} & \cellcolor{green!50}78.26\std{1.52} & \cellcolor{green!50}79.23\std{1.65} & \cellcolor{green!50}85.74\std{1.85} & \cellcolor{green!50}86.32\std{1.48} \\
        & HM-BiTCN & 82.49\std{1.40} & 82.38\std{1.79} & 81.20\std{1.32} & 81.60\std{1.39} & 91.10\std{1.63} & 91.30\std{1.71} \\
        & HM-BiTCN + CIF & \cellcolor{green!50}\textbf{85.16\std{1.55}} & \cellcolor{green!50}84.76\std{1.62} & \cellcolor{green!50}\textbf{85.33\std{1.27}} & \cellcolor{green!50}\textbf{84.82\std{1.49}} & \cellcolor{green!50}\textbf{94.06\std{1.07}} & \cellcolor{green!50}\textbf{94.21\std{0.99}} \\
        \bottomrule
    \end{tabular}}
\end{table}



% 彩色

\begin{table}[htp]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent-TDBRAIN}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
    \midrule
    \multirow{26}{*}
    % {\textbf{TDBrain \\(2-Classes)}} 
    {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{TDBrain} \\ (2-Classes) \\Reproduced} \end{tabular}} 
    \rowcolors{2}{gray!10}{white}
    & Autoformer & 90.38\std{3.03} & 91.16\std{2.42} & 90.38\std{3.03} & 90.31\std{3.09} & 95.83\std{2.14} & 95.43\std{2.31} \\
    & Autoformer + CIF & \cellcolor{green!50}\textbf{93.42\std{2.49}} & \cellcolor{green!50}\textbf{93.71\std{2.27}} & \cellcolor{green!50}\textbf{93.42\std{2.49}} & \cellcolor{green!50}\textbf{93.40\std{2.51}} & \cellcolor{green!50}97.46\std{1.08} & \cellcolor{green!50}97.21\std{1.15} \\
    & Crossformer & 82.15\std{2.60} & 82.81\std{2.11} & 82.15\std{2.60} & 82.04\std{2.70} & 91.20\std{2.23} & 91.47\std{2.16} \\
    & Crossformer + CIF & \cellcolor{green!50}89.40\std{1.26} & \cellcolor{green!50}89.83\std{1.18} & \cellcolor{green!50}89.40\std{1.26} & \cellcolor{green!50}89.37\std{1.27} & \cellcolor{green!50}96.76\std{0.62} & \cellcolor{green!50}96.80\std{0.62} \\
    & FEDformer & 77.60\std{1.23} & 78.25\std{1.52} & 77.60\std{1.23} & 77.48\std{1.19} & 86.31\std{1.23} & 86.48\std{1.36} \\
    & FEDformer + CIF & \cellcolor{green!50}78.87\std{1.94} & \cellcolor{green!50}79.19\std{2.00} & \cellcolor{green!50}78.88\std{1.94} & \cellcolor{green!50}78.82\std{1.94} & \cellcolor{green!50}88.12\std{1.87} & \cellcolor{green!50}88.39\std{1.92} \\
    & Informer & 88.42\std{2.99} & 89.01\std{2.45} & 88.42\std{2.99} & 88.36\std{3.05} & 96.54\std{0.90} & 96.66\std{0.85} \\
    & Informer + CIF & \cellcolor{green!50}89.38\std{1.66} & \cellcolor{green!50}89.71\std{1.37} & \cellcolor{green!50}89.38\std{1.66} & \cellcolor{green!50}89.35\std{1.68} & \cellcolor{green!50}96.92\std{0.66} & \cellcolor{green!50}97.03\std{0.64} \\
    & iTransformer & 74.69\std{1.02} & 74.76\std{1.04} & 74.69\std{1.02} & 74.67\std{1.02} & 83.35\std{1.24} & 83.65\std{1.41} \\
    & iTransformer + CIF & 72.79\std{1.12} & 72.89\std{1.16} & 72.79\std{1.12} & 72.76\std{1.11} & 81.08\std{1.03} & 81.31\std{0.93} \\
    & MTST & 77.67\std{3.58} & 78.97\std{4.37} & 77.67\std{3.58} & 77.45\std{3.55} & 86.47\std{4.84} & 84.99\std{6.43} \\
    & MTST + CIF & \cellcolor{green!50}87.21\std{1.99} & \cellcolor{green!50}87.30\std{2.06} & \cellcolor{green!50}87.21\std{1.99} & \cellcolor{green!50}87.20\std{1.99} & \cellcolor{green!50}94.14\std{1.83} & \cellcolor{green!50}93.24\std{2.63} \\
    & Nonformer & 88.10\std{2.39} & 88.76\std{1.74} & 88.10\std{2.39} & 88.04\std{2.47} & 96.56\std{0.91} & 96.36\std{1.21} \\
    & Nonformer + CIF & 88.00\std{2.06}& \cellcolor{green!50}88.91\std{1.68}& 88.00\std{2.06}& 87.92\std{2.12}& \cellcolor{green!50}97.10\std{1.10}& \cellcolor{green!50}97.17\std{1.09} \\
    & PatchTST & 77.98\std{2.64} & 79.30\std{3.73} & 77.98\std{2.64} & 77.76\std{2.65} & 86.67\std{4.03} & 84.93\std{5.47} \\
    & PatchTST + CIF & \cellcolor{green!50}79.58\std{0.86} & \cellcolor{green!50}80.22\std{0.82} & \cellcolor{green!50}79.58\std{0.86} & \cellcolor{green!50}79.47\std{0.88} & \cellcolor{green!50}87.20\std{1.57} & \cellcolor{green!50}85.81\std{1.17} \\
    & Reformer & 88.50\std{2.30} & 89.01\std{1.80} & 88.50\std{2.30} & 88.45\std{2.35} & 96.10\std{0.63} & 96.19\std{0.55} \\
    & Reformer + CIF & \cellcolor{green!50}89.08\std{1.19} & \cellcolor{green!50}89.47\std{0.70} & \cellcolor{green!50}89.08\std{1.19} & \cellcolor{green!50}89.05\std{1.23} & \cellcolor{green!50}96.88\std{0.35} & \cellcolor{green!50}97.00\std{0.35} \\
    & Transformer & 85.13\std{1.86} & 86.39\std{1.56} & 85.13\std{1.86} & 84.99\std{1.93} & 95.61\std{1.05} & 95.63\std{0.91} \\
    & Transformer + CIF & \cellcolor{green!50}89.96\std{1.57} & \cellcolor{green!50}90.53\std{1.26} & \cellcolor{green!50}89.96\std{1.57} & \cellcolor{green!50}89.92\std{1.60} & \cellcolor{green!50}97.73\std{0.45} & \cellcolor{green!50}97.77\std{0.46} \\
    & Medformer & 88.77\std{1.24} & 88.91\std{1.11} & 88.77\std{1.24} & 88.76\std{1.25} & 96.38\std{0.34} & 96.44\std{0.30} \\
    & Medformer + CIF & \cellcolor{green!50}90.88\std{0.87} & \cellcolor{green!50}90.94\std{0.81} & \cellcolor{green!50}90.88\std{0.87} & \cellcolor{green!50}90.87\std{0.87} & \cellcolor{green!50}97.39\std{0.30} & \cellcolor{green!50}97.46\std{0.28} \\
    % & MedGNN & 82.60\std{0.35} & \textbf{87.70\std{0.22} & 78.93\std{0.09} & 80.25\std{0.16} & 85.93\std{0.26} & - \\
    % & MedGNN + CIC & - & - & - & - & - & - \\
    & HM-BiTCN & 84.90\std{2.60} & 86.02\std{2.00} & 84.90\std{2.60} & 84.76\std{2.74} & 93.94\std{1.92} & 94.20\std{1.85} \\
    & HM-BiTCN + CIF & \cellcolor{green!50}93.13\std{1.41} & \cellcolor{green!50}93.33\std{1.37} & \cellcolor{green!50}93.13\std{1.41} & \cellcolor{green!50}93.12\std{1.42} & \cellcolor{green!50}\textbf{98.62\std{0.66}} & \cellcolor{green!50}\textbf{98.68\std{0.63}} \\
    \bottomrule
\end{tabular}}
\end{table}
\newpage


% 彩色

\begin{table}[htp]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent-ADFTD}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    \textbf{Datasets} & \textbf{Models} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score} & \textbf{AUROC} & \textbf{AUPRC}  \\
    \midrule
    \multirow{26}{*}
    % {\textbf{ADFTD} \\ (3-Classes)} 
        {\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{ADFTD} \\ (3-Classes) \\Reproduced} \end{tabular}} 
    \rowcolors{2}{gray!10}{white}
    & Autoformer & 46.90\std{2.89} & 45.59\std{2.37} & 44.91\std{2.23} & 44.34\std{2.52} & 63.49\std{2.44} & 45.63\std{2.29} \\
    & Autoformer + CIF & 45.92\std{2.78} & 44.81\std{2.44} & 44.66\std{2.25} & 44.26\std{2.38} & 62.69\std{2.21} & 44.93\std{2.68} \\
    & Crossformer & 50.18\std{1.97} & 45.97\std{1.84} & 46.30\std{1.73} & 45.90\std{1.84} & 66.68\std{1.67} & 48.65\std{1.89} \\
    & Crossformer + CIF & \cellcolor{green!50}54.58\std{1.22} & \cellcolor{green!50}47.85\std{0.67} & \cellcolor{green!50}48.96\std{0.89} & \cellcolor{green!50}48.22\std{0.72} & \cellcolor{green!50}69.10\std{1.05} & \cellcolor{green!50}52.23\std{0.98} \\
    & FEDformer & 45.75\std{0.78} & 45.71\std{1.29} & 44.27\std{1.28} & 43.51\std{1.00} & 62.64\std{1.64} & 45.88\std{1.35} \\
    & FEDformer + CIF & \cellcolor{green!50}48.63\std{1.99} & \cellcolor{green!50}46.97\std{1.58} & \cellcolor{green!50}46.87\std{1.63} & \cellcolor{green!50}46.69\std{1.54} & \cellcolor{green!50}65.56\std{2.14} & \cellcolor{green!50}48.30\std{2.30} \\
    & Informer & 48.42\std{1.99} & 46.94\std{1.60} & 46.41\std{0.99} & 45.76\std{0.43} & 65.99\std{1.14} & 47.49\std{1.07} \\
    & Informer + CIF & \cellcolor{green!50}50.12\std{0.66} & \cellcolor{green!50}47.23\std{0.47} & \cellcolor{green!50}46.77\std{0.39} & \cellcolor{green!50}46.62\std{0.38} & 65.13\std{0.52} & 46.84\std{0.54} \\
    & iTransformer & 52.85\std{1.36} & 46.97\std{1.05} & 47.31\std{1.03} & 46.84\std{0.78} & 67.46\std{0.96} & 49.90\std{0.89} \\
    & iTransformer + CIF & 50.76\std{0.50} & \cellcolor{green!50}47.11\std{0.67} & 47.29\std{0.59} & \cellcolor{green!50}47.10\std{0.66} & 67.00\std{0.55} & 49.60\std{0.69} \\
    & MTST & 45.77\std{1.70} & 44.39\std{1.73} & 43.70\std{1.82} & 43.36\std{1.98} & 61.38\std{1.57} & 44.01\std{1.60} \\
    & MTST + CIF & \cellcolor{green!50}46.36\std{0.93} & \cellcolor{green!50}45.04\std{0.65} & \cellcolor{green!50}45.47\std{0.88} & \cellcolor{green!50}44.87\std{0.81} & \cellcolor{green!50}63.57\std{1.24} & \cellcolor{green!50}47.35\std{1.36} \\
    & Nonformer & 50.81\std{1.06} & 48.71\std{1.40} & 48.55\std{1.47} & 48.36\std{1.38} & 66.95\std{1.54} & 48.08\std{1.82} \\
    & Nonformer + CIF & \cellcolor{green!50}51.81\std{2.11} & \cellcolor{green!50}49.93\std{0.81} & \cellcolor{green!50}49.66\std{0.36} & \cellcolor{green!50}49.10\std{0.57} & \cellcolor{green!50}68.59\std{0.60} & \cellcolor{green!50}50.44\std{0.94} \\
    & Reformer & 51.28\std{2.60} & 49.68\std{2.75} & 49.64\std{2.02} & 48.45\std{2.06} & 69.20\std{2.53} & 51.74\std{3.24} \\
    & Reformer + CIF & \cellcolor{green!50}52.50\std{0.91} & \cellcolor{green!50}52.10\std{2.91} & 49.01\std{2.74} & 47.53\std{4.23} & 68.25\std{1.79} & 50.44\std{2.59} \\
    & Transformer & 50.53\std{0.94} & 49.31\std{0.87} & 48.57\std{1.23} & 48.42\std{1.28} & 67.98\std{0.90} & 49.07\std{1.35} \\
    & Transformer + CIF & \cellcolor{green!50}52.84\std{2.50} & \cellcolor{green!50}51.27\std{2.33} & \cellcolor{green!50}51.53\std{2.37} & \cellcolor{green!50}51.10\std{2.21} & \cellcolor{green!50}70.25\std{2.42} & \cellcolor{green!50}52.35\std{2.94} \\
    & Medformer & 53.70\std{1.18} & 51.51\std{1.32} & 50.49\std{1.48} & 50.35\std{1.53} & 70.48\std{1.17} & 50.91\std{1.13} \\
    & Medformer + CIF & \cellcolor{green!50}55.88\std{0.82} & \cellcolor{green!50}51.91\std{1.90} & \cellcolor{green!50}50.80\std{1.63} & 50.29\std{1.92} & 70.45\std{1.33} & \cellcolor{green!50}53.73\std{1.70} \\
    % & MedGNN & 82.60\std{0.35} & \textbf{87.70\std{0.22}} & 78.93\std{0.09} & 80.25\std{0.16} & 85.93\std{0.26} & - \\
    % & MedGNN + CIC & 82.60\std{0.35} & \textbf{87.70\std{0.22}} & 78.93\std{0.09} & 80.25\std{0.16} & 85.93\std{0.26} & - \\
    & HM-BiTCN & 52.05\std{2.22} & 50.45\std{3.00} & 50.40\std{2.55} & 49.48\std{2.70} & 69.43\std{2.84} & 50.99\std{3.15} \\
    & HM-BiTCN + CIF & \cellcolor{green!50}\textbf{58.56\std{0.93}} & \cellcolor{green!50}\textbf{55.65\std{0.81}} & \cellcolor{green!50}\textbf{55.86\std{0.79}} & \cellcolor{green!50}\textbf{55.42\std{0.82}} & \cellcolor{green!50}\textbf{76.07\std{0.59}} & \cellcolor{green!50}\textbf{59.75\std{0.67}} \\
       \bottomrule
\end{tabular}
}
\end{table}



% 变色

\begin{table}[htpt]
\centering
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Independent Setup.} Green cells indicate performance improvement with CIF.}
\label{tab:subject-independent-PTB}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}
    \toprule
    \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPRC}}  \\
    \midrule
    \multirow{26}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{PTB} \\ (2-Classes)} \end{tabular}} 
    \rowcolors{2}{gray!10}{white} % Set row colors (alternating gray and white)
    & \textbf{Autoformer} & 71.99\std{2.74} & 69.60\std{3.85} & 61.50\std{4.23} & 61.43\std{5.07} & 74.29\std{1.89} & 70.26\std{2.00} \\
    & \textbf{Autoformer + CIF} & \cellcolor{green!50}77.71\std{0.63} & \cellcolor{green!50}77.15\std{1.29} & \cellcolor{green!50}70.32\std{1.62} & \cellcolor{green!50}71.77\std{1.60} & \cellcolor{green!50}81.20\std{4.15} & \cellcolor{green!50}78.13\std{4.80} \\
    & \textbf{Crossformer} & 78.06\std{3.44} & 81.53\std{3.13} & 68.62\std{5.63} & 69.76\std{6.53} & 88.31\std{2.07} & 85.81\std{2.43}  \\
    & \textbf{Crossformer + CIF} & \cellcolor{green!50}84.55\std{4.80} & \cellcolor{green!50}85.96\std{3.63} & \cellcolor{green!50}78.64\std{7.49} & \cellcolor{green!50}80.25\std{7.89} & \cellcolor{green!50}92.17\std{2.99} & \cellcolor{green!50}91.16\std{3.70} \\
    & \textbf{FEDformer} & 74.54\std{2.27} & 77.99\std{4.10} & 63.14\std{3.29} & 63.28\std{4.36} & 84.63\std{4.27} & 80.91\std{5.55} \\
    & \textbf{FEDformer + CIF} & \cellcolor{green!50}77.93\std{1.86} & \cellcolor{green!50}80.65\std{3.50} & \cellcolor{green!50}68.59\std{2.20} & \cellcolor{green!50}70.23\std{2.63} & \cellcolor{green!50}86.00\std{3.51} & \cellcolor{green!50}83.42\std{4.76} \\
    & \textbf{Informer} & 79.59\std{0.65} & 83.33\std{0.77} & 70.58\std{0.95} & 72.58\std{1.08} & 92.77\std{0.48} & 90.89\std{0.57} \\
    & \textbf{Informer + CIF} & \cellcolor{green!50}83.63\std{2.32} & \cellcolor{green!50}85.31\std{1.80} & \cellcolor{green!50}77.28\std{3.67} & \cellcolor{green!50}79.37\std{3.45} & \cellcolor{green!50}93.87\std{0.48} & \cellcolor{green!50}92.29\std{0.63}  \\
    & \textbf{iTransformer} & 83.43\std{1.19} & 88.06\std{1.47} & 75.64\std{1.55} & 78.29\std{1.70} & 91.38\std{1.41} & 91.08\std{1.30}  \\
    & \textbf{iTransformer + CIF} & 81.62\std{2.96} & 87.48\std{2.03} & 72.74\std{4.41} & 74.99\std{4.91} & 90.25\std{3.29} & 89.80\std{3.28} \\
    & \textbf{MTST} & 75.53\std{2.45} & 78.72\std{1.87} & 64.78\std{4.06} & 65.30\std{4.81} & 87.76\std{4.09} & 83.60\std{3.92}  \\
    & \textbf{MTST + CIF} & \cellcolor{green!50}81.80\std{1.60} & \cellcolor{green!50}84.19\std{2.05} & \cellcolor{green!50}74.28\std{2.05} & \cellcolor{green!50}76.52\std{2.25} & \cellcolor{green!50}91.30\std{2.48} & \cellcolor{green!50}88.41\std{3.30} \\
    & \textbf{Nonformer} & 78.93\std{1.46} & 82.48\std{1.53} & 69.68\std{2.15} & 71.50\std{2.56} & 90.54\std{0.59} & 87.78\std{1.46}  \\
    & \textbf{Nonformer + CIF} & 71.89\std{3.81} & 71.80\std{4.58} & 69.44\std{3.56} & 69.74\std{3.84} & 70.55\std{2.96} & 70.78\std{4.08} \\
    & \textbf{PatchTST} & 75.28\std{2.44} & 77.05\std{2.44} & 64.86\std{4.05} & 65.41\std{5.28} & 88.11\std{2.59} & 82.65\std{2.87} \\
    & \textbf{PatchTST + CIF} & \cellcolor{green!50}80.80\std{1.90} & \cellcolor{green!50}82.46\std{1.75} & \cellcolor{green!50}73.23\std{2.81} & \cellcolor{green!50}75.24\std{2.95} & \cellcolor{green!50}92.45\std{0.91} & \cellcolor{green!50}88.23\std{1.61} \\
    & \textbf{Reformer} & 78.11\std{1.65} & 82.70\std{0.80} & 68.17\std{2.68} & 69.68\std{3.34} & 90.77\std{1.56} & 88.14\std{1.20}  \\
    & \textbf{Reformer + CIF} & \cellcolor{green!50}81.95\std{2.09} & \cellcolor{green!50}84.63\std{1.07} & \cellcolor{green!50}74.44\std{3.53} & \cellcolor{green!50}76.55\std{3.64} & \cellcolor{green!50}93.36\std{0.87} & \cellcolor{green!50}91.53\std{1.05} \\
    & \textbf{Transformer} & 76.43\std{1.98} & 81.25\std{1.15} & 65.64\std{3.29} & 66.44\std{4.39} & 90.21\std{1.24} & 87.28\std{1.49} \\
    & \textbf{Transformer + CIF} & \cellcolor{green!50}78.80\std{2.44} & \cellcolor{green!50}82.45\std{2.36} & \cellcolor{green!50}69.42\std{3.62} & \cellcolor{green!50}71.10\std{4.33} & \cellcolor{green!50}92.50\std{1.17} & \cellcolor{green!50}89.07\std{1.39} \\
    & \textbf{Medformer}  & 80.99\std{0.75} & 83.01\std{0.72} & 73.35\std{1.16} & 75.47\std{1.21} & 93.10\std{1.18} & 90.69\std{1.04} \\
    & \textbf{Medformer + CIF} & 78.74\std{0.64} & \cellcolor{green!50}81.11\std{0.84} & \cellcolor{green!50}75.40\std{0.66} & \cellcolor{green!50}76.31\std{0.71} & 83.20\std{0.91} & 83.66\std{0.92} \\
    % & \textbf{MedGNN} & 82.60\std{0.35} & \textbf{87.70\std{0.22}} & 78.93\std{0.09} & 80.25\std{0.16} & 85.93\std{0.26} & - \\
    % & \textbf{MedGNN + CIC} &  &  & &  &  & - \\
    & \textbf{HM-BiTCN} & 81.87\std{1.87} & 86.50\std{1.24} & 73.49\std{2.90} & 75.84\std{3.20} & 94.20\std{0.29} & 93.04\std{0.45} \\
    & \textbf{HM-BiTCN + CIF}   & \cellcolor{green!50}\textbf{88.29\std{1.45}} & \cellcolor{green!50}\textbf{90.66\std{1.48}} & \cellcolor{green!50}\textbf{83.21\std{2.02}} & \cellcolor{green!50}\textbf{85.59\std{1.96}} & \cellcolor{green!50}\textbf{94.28\std{0.93}} & \cellcolor{green!50}\textbf{93.78\std{1.11}}  \\
    \bottomrule
\end{tabular}
}
\end{table}



==> table/subject.tex <==


\begin{table}[]
\centering
% \scriptsize
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Dependent Setup.} The training, validation, and test sets are split based on samples according to a predetermined ratio. Results of the ADFTD dataset under this setup are presented here.
}
\label{tab:subject-dependent}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}


    \toprule
    \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPRC}} \\


    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{ADFTD} \\ (3-Classes)} \end{tabular}} %&
    & \textbf{Autoformer} & 87.83\std{1.62} & 87.63\std{1.66} & 87.22\std{1.97} & 87.38\std{1.79} & 96.59\std{0.88} & 93.82\std{1.64} \\
    & \textbf{Crossformer} & 89.35\std{1.32} & 89.00\std{1.44} & 88.79\std{1.37} & 88.88\std{1.40} & 97.52\std{0.58} & 95.45\std{1.03} \\
    & \textbf{FEDformer} & 77.63\std{2.37} & 76.76\std{2.17} & 76.68\std{2.48} & 76.60\std{2.46} & 91.67\std{1.34} & 84.94\std{2.11} \\
    & \textbf{Informer} & 90.93\std{0.90} & 90.74\std{0.71} & 90.50\std{1.14} & 90.60\std{0.94} & 98.19\std{0.27} & 96.51\std{0.49} \\
    & \textbf{iTransformer} & 64.90\std{0.25} & 62.53\std{0.27} & 62.21\std{0.26} & 62.25\std{0.33} & 81.52\std{0.29} & 68.87\std{0.49} \\
    & \textbf{MTST}  & 65.08\std{0.69} & 63.85\std{0.80} & 62.71\std{0.64} & 63.03\std{0.58} & 81.36\std{0.56} & 69.34\std{0.89} \\
    & \textbf{Nonformer}  & 96.12\std{0.47} & 95.94\std{0.56} & 95.99\std{0.38} & 95.96\std{0.47} & 99.59\std{0.09} & 99.08\std{0.16} \\
    & \textbf{PatchTST}  & 66.26\std{0.40} & 65.08\std{0.41} & 64.97\std{0.51} & 64.95\std{0.42} & 83.07\std{0.45} & 71.70\std{0.61} \\
    & \textbf{Reformer}  & 91.51\std{1.75} & 91.15\std{1.79} & 91.65\std{1.56} & 91.14\std{1.83} & 98.85\std{0.35} & 97.88\std{0.60} \\
    & \textbf{Transformer}  & 97.00\std{0.43} & 96.87\std{0.53} & 96.86\std{0.36} & 96.86\std{0.44} & 99.75\std{0.04} & 99.42\std{0.07} \\
    & \textbf{Medformer (Ours)}  & \textbf{97.62\std{0.34}} & \textbf{97.53\std{0.33}} & \textbf{97.48\std{0.40}} & \textbf{97.50\std{0.36}} & \textbf{99.83\std{0.05}} & \textbf{99.62\std{0.12}} \\



\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}


==> table/subject_reproduce.tex <==


\begin{table}[ht]
\centering
% \scriptsize
\def\arraystretch{1.0}
\caption{\textbf{Results of Subject-Dependent Setup.} The training, validation, and test sets are split based on samples according to a predetermined ratio. Results of the ADFTD dataset under this setup are presented here.
}
\label{tab:subject-dependent_reproduce}
\resizebox{\textwidth}{!}{%
\begin{tabular}{clcccccc}


    \toprule
    % \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy}} & \multicolumn{1}{c}{\textbf{Precision}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1 score}} & \multicolumn{1}{c}{\textbf{AUROC}} & \multicolumn{1}{c}{\textbf{AUPRC}} \\
      \textbf{Datasets} & \textbf{Models} & \multicolumn{1}{c}{\textbf{Accuracy $\uparrow$}} & \multicolumn{1}{c}{\textbf{Precision $\uparrow$}} & \multicolumn{1}{c}{\textbf{Recall $\uparrow$}} & \multicolumn{1}{c}{\textbf{F1 score $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUROC $\uparrow$}} & \multicolumn{1}{c}{\textbf{AUPRC $\uparrow$}} \\


    \midrule
    \multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}\;\makecell{\textbf{ADFTD} \\ (3-Classes) \\Reproduced} 
    \end{tabular}} %&
    
    & \textbf{Autoformer}~\cite{wu2021autoformer} & 87.79\std{2.87}& 87.63\std{2.95}& 86.84\std{3.10}& 87.17\std{3.05}& 96.45\std{1.15}& 93.52\std{2.05} \\
& \textbf{Crossformer}~\cite{zhang2022crossformer} & 89.27\std{1.19}& 88.98\std{1.27}& 88.61\std{1.35}& 88.77\std{1.29}& 97.53\std{0.48}& 95.47\std{0.87} \\
    & \textbf{FEDformer}~\cite{zhou2022fedformer} & 77.55\std{2.42}& 76.71\std{2.14}& 76.46\std{2.52}& 76.44\std{2.52}& 91.66\std{1.36}& 84.99\std{2.15}  \\
    & \textbf{Informer}~\cite{zhou2021informer} & 91.72\std{0.13}& 91.50\std{0.16}& 91.36\std{0.21}& 91.42\std{0.14}& 98.40\std{0.07}& 96.92\std{0.11} \\
    & \textbf{iTransformer}~\cite{liu2023itransformer} & 64.60\std{0.77}& 62.22\std{0.64}& 61.95\std{0.35}& 61.87\std{0.41}& 81.46\std{0.29}& 68.81\std{0.39} \\
    & \textbf{MTST}~\cite{zhang2024multi} & 65.43\std{0.79}& 64.47\std{0.65}& 63.49\std{0.55}& 63.71\std{0.55}& 81.67\std{0.51}& 69.74\std{0.69} \\
    & \textbf{Nonformer}~\cite{liu2022non} & 96.00\std{0.72}& 95.72\std{0.80}& 95.90\std{0.69}& 95.81\std{0.75}& 99.56\std{0.13}& 99.02\std{0.23} \\
    & \textbf{PatchTST}~\cite{nie2022time} & 66.55\std{0.48}& 65.61\std{0.60}& 65.26\std{0.78}& 65.26\std{0.60}& 83.27\std{0.33}& 71.96\std{0.44} \\
    & \textbf{Reformer}~\cite{kitaev2019reformer} & 90.74\std{2.18}& 90.87\std{2.15}& 90.61\std{2.01}& 90.44\std{2.25}& 98.69\std{0.50}& 97.57\std{0.85} \\
    & \textbf{Transformer}~\cite{vaswani2017attention} & 96.62\std{0.54}& 96.46\std{0.54}& 96.45\std{0.59}& 96.45\std{0.56}& 99.69\std{0.08}& 99.31\std{0.13} \\
    & \textbf{Medformer}~\cite{wang2024medformer} & 95.76\std{1.03}& 95.54\std{1.10}& 95.62\std{1.05}& 95.58\std{1.08}& 99.53\std{0.18}& 99.09\std{0.36}  \\

    & \textbf{Medformer + CIF}  & 98.87\std{0.26}& 98.77\std{0.27}& 98.86\std{0.27}& 98.81\std{0.27}& 99.96\std{0.01}& 99.92\std{0.03} \\

    & \textbf{MedGNN}~\cite{fan2025medgnn} & 99.44\std{0.21}& 99.43\std{0.21}& 99.41\std{0.22}& 99.42\std{0.21}& 99.98\std{0.01}&\textbf{99.97\std{0.01}} \\

% & \textbf{MedGNN + CIC} & 99.60\std{0.09}& 99.60\std{0.11}& 99.58\std{0.09}& 99.59\std{0.10}& 99.99\std{0.01}& 99.97\std{0.01} \\

& \textbf{MedGNN + CIF} & \textbf{99.60\std{0.09}}& \textbf{99.60\std{0.11}}& \textbf{99.58\std{0.09}}& \textbf{99.59\std{0.10}}& \textbf{99.99\std{0.01}}& \textbf{99.97\std{0.01}} \\
\bottomrule
\end{tabular}
}
\end{table}

